Training Set Camouflage

We introduce a form of steganography in the domain of machine learning which we call training set camouflage. Imagine Alice has a training set on an illicit machine learning classification task. Alice wants Bob (a machine learning system) to learn the task. However, sending either the training set or the trained model to Bob can raise suspicion if the communication is monitored. Training set camouflage allows Alice to compute a second training set on a completely different -- and seemingly benign -- classification task. By construction, sending the second training set will not raise suspicion. When Bob applies his standard (public) learning algorithm to the second training set, he approximately recovers the classifier on the original task. Training set camouflage is a novel form of steganography in machine learning. We formulate training set camouflage as a combinatorial bilevel optimization problem and propose solvers based on nonlinear programming and local search. Experiments on real classification tasks demonstrate the feasibility of such camouflage.

==> arxiv_Paper (copy)/clean_run_exp.tex <==
We investigated the effectiveness of training set camouflage through empirical experiments on real world datasets. 
Our results show that camouflage works on a variety of image and text classification tasks: 
Bob can perform well on the secret task after training on the camouflaged training set, and the camouflaged training set passes Eve's test undetected.
We start by discussing the three agents.

\textbf{Bob}.  We considered the logistic regression learning algorithm for Bob.
Logistic regression is a popular learner and is regularly used in practice. 
Bob set the weight of the regularization parameter to $1$. 

\textbf{Eve}.
%The application of training set camouflage framework is independent of Eve's choice of detection function.
The training set camouflage framework is general with respect to Eve's detection function.
For our experiments we used Maximum Mean Discrepancy  ({\mmd})~\cite{gretton2012kernel} as the core of Eve's detection function.
We used {\mmd} as it is a popular and widely used two-sample test~\cite{dziugaite2015training}.
Unfortunately {\mmd} cannot be directly applied to the camouflage framework as its application requires that the two samples have the same size.
We introduce {\mmd} and how Eve used it in Appendix A.
The level-$\alpha$ for this detection function was set to $0.05$ (i.e., the probability of incorrectly rejecting a benign training set is 5\%). 

\textbf{Alice}. 
We considered three different Alices. Each of them used one of the proposed solvers.
For each secret task, Alice had access to multiple camouflage candidate tasks.
Alice can run her solver on each of these tasks separately and then select the best one, but this would be time consuming and thus instead she started by identifying a suitable camouflage task.
For this purpose, all three Alices used uniform sampling (as this is the easiest algorithm to implement, and makes the weakest assumptions) with a search budget of $80,000$ (divided equally among candidate tasks).
This meant that Alice stopped after training the logistic regression learner $80,000$ times.
For each candidate task Alice identified a training set using this budget.
Then she selected the best task (as her cover task) based on the loss on the secret set.

Next, all three Alices used their respective solvers (NLP, beam search and uniform sampling) to find a camouflaged training set.
We assumed that all of them were allotted a fixed amount of time for this purpose.
This time was set as the time required to run the NLP solver. %with an additional two hours.
%The extra two hours were allotted as in some cases the NLP solver finished within a few seconds.
%This time is not enough for the other two solvers to find any useful solution.

The Alice who used the NLP solver seeded the solver with the camouflaged training set found during the candidate task identification phase.
The Alice who used the beam search solver performed random restarts each with a per-restart budget of $B/R = 16,000$.
Here the width of the beam was $w=10$ and for each training set in the beam, $50$ randomly selected neighbors were evaluated during each iteration.
It should be noted that both beam search and uniform sampling are stochastic in nature.
We run the Alices who used these solvers five times. 
We then report the average.
Alice constructed camouflaged training sets of size $m=2, 20$ and $50$, $100$ and $500$, and set the loss $\ell$ to logistic loss with natural logarithm.
All experiments were run on an Intel(R) Core(TM) i7-7700T CPU @2.90GHz machine, using one thread.


%Alice constructed camouflaged training sets of size $m=20$ and $50$.
%The construction took place in two phases.
%In the first phase, Alice identified a suitable camouflage task from several candidates.
%During this phase, she used uniform sampling with a search budget of $80,000$.
%This meant that Alice stopped the search after training the logistic regression learner $80,000$ times.
%In the second phase, Alice used all three solvers to find a camouflaged training set.
%We assume that Alice is allotted a fixed amount of time for this purpose.
%This time is set as the time required to run the NLP solver (seeded with the camouflaged training set found during the first phase) with an additional two hours.
%For this NLP solver, Alice evaluates a further $m$ training sets as part of the rounding procedure.
%Let $I$ and $N$ identify the index vector of all instances in the initial dataset and all other instances in the camouflage pool respectively. 
%Also let, $I'$ and $N'$ represent the sorted sequence of $I$ and $N$ such that $b_{I'_i} \ge b_{I'_i+1}$ and $b_{I'_i} \ge b_{I'_i+1}$. Now we define,
%$T_c=[I'_1,I'_2,\ldots,I'_{m-c},N'_1,N'_2,\ldots,N'_c]$.  
%Here $c\in\mathbb{Z}: c\in[0,m]$. 
%Thus $T_0=I'$ and $T_m=[N'_1,N'_2,\ldots,N'_m]$.
%Alice evaluates the training sets $\cand_{T_c}$ for all values of $c$. 
%Note that she does not need to re-evaluate $T_0$. Thus the camouflaged training set found by using the NLP solver is:
%\begin{align}
%\argmin_{c\in\mathbb{Z}: c\in[0,m]}& ~~&&\frac{1}{\vert \val \vert} \sum_{(\tx, \ty)\in \val}\tloss(\hat{\theta}, \tx, \ty)\nonumber\\
%\text{s.t.}& ~~&&\hat{\theta} = \argmin_{\theta \in \Theta} \sum_{(\bfx, y)\in\cand_{T_c}} \closs(\theta, \bfx, y) + \frac{\lambda}{2} \Vert \theta \Vert^2\nonumber\\
%& &&\suspicion(\cand,\cand_{T_c}) < 0
%\end{align}
%For beam search Alice performs random restarts each with a budget of $16,000$.
%Here the size of the beam was $10$ and for each training set in the beam, $50$ randomly selected neighbors were evaluated during each iteration.
%It should be noted that both beam search and uniform sampling are stochastic in nature.
%Thus we repeat these solvers $5$ times and report the average.
%Alice set the loss $\ell$ to logistic loss.
%All experiments were run on an Intel(R) Core(TM) i7-7700T CPU @2.90GHz machine.

\textbf{Evaluation metrics}.
As is standard to estimate generalization performance of a learned model, we used a separate test set, generated from the same distribution as the secret set $D_S$ and not known to any agent, to estimate Bob's generalization error when trained on Alice's camouflaged training set $D$.
We compare these values to two additional quantities:
(``random'') when Bob is trained on a uniform sample of size $m$ from the cover data distribution, which we expect to perform poorly; and 
(``oracle'') when Bob is trained directly on Alice's secret set $D_S$, ignoring Eve's presence.
The oracle gives us an estimate on how much performance Bob is losing due to using the camouflage framework to fool Eve.

\subsection{Datasets}
We performed experiments for four secret tasks: WM (CIFAR-100~\cite{krizhevsky2009learning}), GP (OpenImages~\cite{openimages}), CA (20-newsgroups~\cite{joachims1996probabilistic}) and DR (All The News dataset~\cite{allthenews2017}).
The two letters in the acronym represent the two classes in the corresponding task (see Table~\ref{tab:dataSum}).
The first two tasks were image classification while the remaining two were text classification.
%We select candidate cover tasks that are confusable and/or neutral.
For the image tasks we selected eight candidate cover tasks. 
Six of them were from the MNIST handwritten digits: 17, 71, 25, 52, 69 and 96.
The other two were from the CIFAR-100 dataset: OA and AO.
Similarly for the text tasks we also selected eight candidate cover tasks.
All of them were from the 20-newsgroups dataset: BH, HB, IM, MI, AM, MA, MX and XM.
As before the acronyms here represent the class names.

\begin{table}
	\centering
	\caption{Summary of secret sets and camouflage pools.}~\label{tab:dataSum}
	%\resizebox{0.8\textwidth}{!}{
		\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		\textbf{Dataset} & \textbf{Type} & \textbf{\# Features} & \textbf{class 1} & \textbf{class 2} & \textbf{\# class 1} & \textbf{\# class 2} \\\hline
		WM & Image & 2048 & \textbf{w}oman & \textbf{m}an & 500 & 500 \\\hline
		GP & Image & 2048 & hand\textbf{g}un & \textbf{p}hone & 400 & 400 \\\hline
		CA & Text & 300 & \textbf{c}hristian & \textbf{a}theist & 599 & 480 \\\hline
		DR & Text & 300 & \textbf{d}emocratic & \textbf{r}epublican & 800 & 800 \\\hline
		17 & Image & 2048 & digit \textbf{1} & digit \textbf{7} & 600 & 600 \\\hline
		25 & Image & 2048 & digit \textbf{2} & digit \textbf{5} & 600 & 600 \\\hline
		69 & Image & 2048 & digit \textbf{6} & digit \textbf{8} & 600 & 600 \\\hline
		OA & Image & 2048 & \textbf{o}range & \textbf{a}pple & 600 & 600 \\\hline
		BH & Text & 300 & \textbf{b}aseball & \textbf{h}ockey & 994 & 999 \\\hline
		IM & Text & 300 & \textbf{i}bm & \textbf{m}ac & 982 & 963 \\\hline
		AM & Text & 300 & \textbf{a}utos & \textbf{m}otorcycles & 990 & 996 \\\hline
		MX & Text & 300 & \textbf{m}s-windows & windows \textbf{x} &985 & 988 \\\hline
	\end{tabular}
	%}
\end{table}

For images we used ResNet~\cite{he2016deep} to generate feature vectors of dimension $2048$. 
For this purpose we removed the output layer and used the values found in the penultimate layer of the network.
For text we used Word2Vec~\cite{mikolov2013efficient} to generate feature vectors of dimension $300$ by averaging over the word vectors in an article.
We also removed punctuation and stop words before generating the word vectors.
A summary of the secret sets and camouflage pools can be found in Table~\ref{tab:dataSum}. As mentioned previously, we kept a held out test set for each of the secret tasks. The number of class 1 and class 2 instances were 100/100, 100/100, 398/319 and 200/200 respectively for WM, GP, CA and DR.
Here the two numbers (num1/num2) represent the number of instances in class1 and class2 respectively.

\begin{table}[!htb]
	\centering
	\caption{Logistic loss ($\frac{1}{|D_S|}\sum_{(\tx,\ty)\in D_S}\log(1+\exp(-\ty w^\top\tx))$) after performing Uniform Sampling search with search budget $10,000$ for image secret tasks. The best results for each secret task is shown in bold.}~\label{tab:imageCandSelect}
	%\resizebox{0.8\textwidth}{!}{
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
		\hline
		m & \backslashbox{Secret}{Camouflage}
		&\makebox[2em]{17}&\makebox[2em]{71}
		&\makebox[2em]{25}&\makebox[2em]{52} &\makebox[2em]{69}&\makebox[2em]{96}
		&\makebox[2em]{OA}&\makebox[2em]{AO}\\\hline 
		%& 17 & 71 & 25 & 52 & 69 & 96 & OA & AO \\\hline
		2 & WM & $0.671$ & $0.631$ & $0.643$ & $0.638$ & $0.671$ & $0.640$ & $\mathbf{0.606}$ & $0.647$    \\\cline{2-10}
		& GP & $0.481$ & $0.541$ & $0.458$ & $\mathbf{0.443}$ & $0.516$ & $0.463$ & $0.541$ & $0.558$ \\\hline
		20 &WM & $0.790$ & $0.611$ & $0.672$ & $0.688$ & $0.798$ & $0.679$ & $\mathbf{0.584}$ & $0.731$ \\\cline{2-10}
		& GP & $0.480$ & $0.510$ & $0.433$ & $0.390$ & $0.632$ & $\mathbf{0.337}$ & $0.510$ & $0.531$ \\\hline
		50 & WM & $0.874$ & $0.614$ & $0.705$ & $0.772$ & $1.116$ & $0.802$ & $\mathbf{0.606}$ & $0.856$ \\\cline{2-10}
		& GP & $0.565$ & $0.479$ & $0.473$ & $\mathbf{0.387}$ & $1.047$ & $0.421$ & $0.479$ & $0.506$   \\\hline
		100 & WM & $0.939$ & $0.651$ & $0.796$ & $0.868$ & $1.441$ & $1.080$ & $\mathbf{0.620}$ & $0.907$ \\\cline{2-10}
		& GP & $0.589$ & $0.469$ & $0.639$ & $\mathbf{0.439}$ & $1.157$ & $0.530$ & $0.0.970$ & $0.538$  \\\hline
		500 & WM & $1.193$ & $0.794$ & $1.107$ & $1.190$ & $2.688$ & $1.988$ & $\mathbf{0.705}$ & $1.283$    \\\cline{2-10}
		& GP & $0.955$ & $\mathbf{0.577}$ & $1.449$ & $0.714$ & $1.795$ & $0.862$& $1.416$ & $0.800$   \\\hline
	\end{tabular}
	%}
\end{table}


Alice first selected a suitable camouflage task for each of the secret tasks.
For each candidate task she used a search budget of $10,000$ (for a total of $80,000$ budget).
The results of this phase are shown in Table~\ref{tab:imageCandSelect} and \ref{tab:textCandSelect}.
The selected camouflage tasks are shown in Table~\ref{tab:tasks}.
It should be noted that the logistic error reported in the tables are large ($>0.693$) in some cases indicating that some of these cover tasks will perform worse than random chance on secret tasks.
However, this was not true for the selected cover tasks.
%Similarly for $m=50$, the selected camouflaged tasks were OA, 52, HB and BH respectively.
The top three camouflaged training sets for GP ($m=20$) identified during this phase are shown in Figure~\ref{fig:candidateCover}.

\begin{table}[!htb]
	\centering
	\caption{Logistic loss after performing Uniform Sampling search with search budget $10,000$ for text secret tasks. The best results for each secret task is shown in bold.}~\label{tab:textCandSelect}
	%\resizebox{0.8\textwidth}{!}{
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
		\hline
		m & \backslashbox{Secret}{Camouflage}
		&\makebox[2em]{BH}&\makebox[2em]{HB}
		&\makebox[2em]{IM}&\makebox[2em]{MI} &\makebox[2em]{AM}&\makebox[2em]{MA}
		&\makebox[2em]{MX}&\makebox[2em]{XM}\\\hline 
		%& 17 & 71 & 25 & 52 & 69 & 96 & OA & AO \\\hline
		2 & CA & $0.6845$ & $0.6846$ & $0.6868$ & $0.6862$ & $0.6861$ & $0.6862$ & $0.6844$ & $\mathbf{0.6843}$ \\\cline{2-10}
		& DR & $0.6889$ & $\mathbf{0.6886}$ & $0.6891$ & $0.6893$ & $0.6888$ & $0.6887$ & $0.6890$ & $0.6894$ \\\hline
		20 & CA & $\mathbf{0.672}$ & $0.673$ & $0.676$ & $0.675$ & $0.676$ & $0.674$ & $0.675$ & $0.675$ \\\cline{2-10}
		& DR & $\mathbf{0.681}$ & $0.684$ & $0.682$ & $0.683$ & $0.682$ & $0.682$ & $0.682$ & $0.683$ \\\hline
		50 & CA & $0.671$ & $\mathbf{0.669}$ & $0.672$ & $0.671$ & $0.674$ & $0.670$ & $0.671$ & $0.671$    \\\cline{2-10}
		& DR & $\mathbf{0.677}$ & $0.681$ & $0.679$ & $0.680$ & $0.678$ & $0.680$ & $0.683$ & $0.679$     \\\hline
		100 & CA & $0.669$ & $0.668$ & $0.669$ & $0.665$ & $0.673$ & $\mathbf{0.661}$ & $0.667$ & $0.668$ \\\cline{2-10}
		& DR & $0.6764$ & $0.6794$ & $0.6791$ & $0.6773$ & $\mathbf{0.6763}$ & $0.6798$ & $0.6787$ & $0.6782$  \\\hline
		500 & CA & $0.677$ & $0.677$ & $0.667$ & $0.678$ & $0.698$ & $\mathbf{0.661}$ & $0.670$ & $0.668$  \\\cline{2-10}
		& DR & $0.685$ & $0.689$ & $0.689$ & $\mathbf{0.681}$ & $0.696$ & $0.698$ & $0.687$ & $0.682$  \\\hline
	\end{tabular}
	%}
\end{table}

\begin{table}
	\centering
	\caption{Selected camouflage tasks}\label{tab:tasks}
	\begin{tabular}{|c|c|c|c|c|c|}
		\hline
		Secret Task & $m=2$ & $m=20$ & $m=50$ & $m=100$ & $m=500$\\\hline
		WM & OA & OA & OA & OA & OA\\\hline
		GP & 52 & 96 & 52 & 52 & 71 \\\hline
		CA & XM & BH & HB & MA & MA \\\hline
		DR & HB & BH & BH & AM & MI \\\hline
	\end{tabular}
\end{table}

\begin{figure}[!htb]
	\centering
	\begin{subfigure}[t]{0.85\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/openimages_sample.pdf}
		\caption{Samples from the secret task Handgun vs. Phone (GP)}~\label{fig:GP}
	\end{subfigure}
	
	\begin{subfigure}[t]{0.85\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/GP96.pdf}
		\caption{Camouflaged training set using 9 vs. 6}~\label{fig:GP96}
	\end{subfigure}
	
	\begin{subfigure}[t]{0.85\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/GP52.pdf}
		\caption{Camouflaged training set using 5 vs 2}~\label{fig:GP52}
	\end{subfigure}
	\begin{subfigure}[t]{0.85\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/GP25.pdf}
		\caption{Camouflaged training set using 2 vs. 5}~\label{fig:GP25}
	\end{subfigure}
	\caption{Samples of GP secret set, and the top three camuflaged training set found during the candidate selection phase for $m=20$.}~\label{fig:candidateCover}
\end{figure}

\begin{table}[htb]
	\centering
	\caption{NLP solver run times}\label{tab:runtimes}
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
			\hline
			\multicolumn{2}{|c|}{$m=2$} & \multicolumn{2}{c|}{$m=20$} & \multicolumn{2}{c|}{$m=50$} & \multicolumn{2}{c|}{$m=100$} & \multicolumn{2}{c|}{$m=500$} \\\hline
			Dataset & Time (s) & Dataset & Time (s) & Dataset & Time (s) & Dataset & Time (s) & Dataset & Time (s) \\\hline
			WMOA & 23363 & WMOA & 29150 & WMOA & 39656 & WMOA & 32186 & WMOA & 56375 \\\hline
			GP52 & 33763 & GP96 & 65697 & GP52 & 171637 & GP52 & 161259 & GP71 & 49354 \\\hline
			CAXM & 48 & CABH & 50 & CAHB & 126 & CAMA & 86 & CAMA & 194 \\\hline
			DRHB & 44 & DRBH & 57 & DRBH & 193 & DRAM & 141 & DRMI & 205 \\\hline
		\end{tabular}
	}
\end{table}


\begin{figure}
	\centering
	\begin{subfigure}[t]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{clean_run_figures/lr_01_2_same.pdf}
		\caption{$m=2$}		
	\end{subfigure}
	\begin{subfigure}[t]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{clean_run_figures/lr_01_20_same.pdf}
		\caption{$m=20$}		
	\end{subfigure}
	
	\begin{subfigure}[t]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{clean_run_figures/lr_01_50_same.pdf}
		\caption{$m=50$}		
	\end{subfigure}
	\begin{subfigure}[t]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{clean_run_figures/lr_01_100_same.pdf}
		\caption{$m=50$}		
	\end{subfigure}
	
	\begin{subfigure}[t]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{clean_run_figures/lr_01_500_same.pdf}
		\caption{$m=50$}		
	\end{subfigure}
	\caption{Test error rates found by solving the camouflage framework. We also show random and oracle error for comparison. Error bars are also shown. All three solvers were run for the same amount of time.}~\label{fig:lr_results_same}
\end{figure}

\begin{figure}
	\centering
	\begin{subfigure}[t]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{clean_run_figures/lr_01_2_extended.pdf}
		\caption{$m=2$}		
	\end{subfigure}
	\begin{subfigure}[t]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{clean_run_figures/lr_01_20_extended.pdf}
		\caption{$m=20$}		
	\end{subfigure}
	
	\begin{subfigure}[t]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{clean_run_figures/lr_01_50_extended.pdf}
		\caption{$m=50$}		
	\end{subfigure}
	\begin{subfigure}[t]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{clean_run_figures/lr_01_100_extended.pdf}
		\caption{$m=50$}		
	\end{subfigure}
	
	\begin{subfigure}[t]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{clean_run_figures/lr_01_500_extended.pdf}
		\caption{$m=50$}		
	\end{subfigure}
	\caption{Test error rates found by solving the camouflage framework. We also show random and oracle error for comparison. Error bars are also shown. The Beam Search and Uniform Search solvers were run for an additional two hours more than the NLP solver run time.}~\label{fig:lr_results_extended}
\end{figure}


\subsection{Results}
The run times for the NLP solver are presented in Table~\ref{tab:runtimes}.
It can be seen from the table that due to the high dimensionality, the NLP solver takes a much longer time to find a solution for the image tasks.
We present our results for all three solvers in Figure~\ref{fig:lr_results_same} and Figure~\ref{fig:lr_results_extended}. %and \ref{fig:lr_results_extended}.
Figure~\ref{fig:lr_results_same} shows the results when all three Alices run their solvers for the same amount of time.
In Figure~\ref{fig:lr_results_extended} we show the results when Beam Search and Uniform Search solvers are run for an additional two hours more than the NLP solver run time.
For the text secret tasks, Alice could not find a better camouflaged training set using either beam search or uniform sampling than the one found during the initial run of uniform sampling (with a total budget of 80,000).
To explore the sensitivity of beam search and uniform sampling regarding the time budget, we ran both solvers for an additional two hours.
But the results only improved marginally (Figure~\ref{fig:lr_results_extended}).
%Even with the added two hours the solutions did not improve by much (Figure~\ref{fig:lr_results_extended}).
We observe that Alice, using any of the three solvers can find much better camouflage training sets than random and in many cases approach oracle performance.
Note that Alice's solutions do not trigger Eve's suspicion function.
This shows that such subterfuges are plausible in practice and can actually yield good results from Alice's point of view.
We note that Alice yields the best results when $m=50$ and $m=500$ respectively for image and text tasks in most of the experiments. 
But this may not hold for larger values of $m$ e.g., when $m$ is equal to the size of the camouflage pool.
We plan to run further experiments to understand the effect of $m$.

Figure~\ref{fig:example} shows the result of WMOA when Bob's learner is logistic regression and the solver is NLP $(m=20)$.
Visually, the camouflaged training set $D$ bears no resemblance to the secret training set $D_S$.
This is true for the text camouflage experiments as well, where articles in the camouflaged training sets have no obvious semantic connection to the secret task. 
See Table~\ref{tab:CABH} for results on the text experiment CABH.
This is indeed bad news for human Eves: not only did camouflage fooled MMD detector, it will also likely fool human inspectors.


\begin{table}[htb]
	\centering
	
	\caption{Camouflage results for the CABH experiment with $m=20$ for the NLP solver}
	\label{tab:CABH}
	
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{|l|l|l|l|}
			\hline
			\multicolumn{2}{|c|}{\textbf{Sample of Secret Set}} & \multicolumn{2}{|c|}{\textbf{Sample of Camouflaged Training Set}} \\\hline
			\multicolumn{1}{|c|}{\textbf{Class}} & \multicolumn{1}{|c|}{\textbf{Article}} & \multicolumn{1}{|c|}{\textbf{Class}} & \multicolumn{1}{|c|}{\textbf{Article}} \\\hline
			Christianity & $\ldots$Christ that often causes christians to be very & Baseball & $\ldots$Boys, hats off to any Cubs fan who can actually\\ 
			&  critical of themselves and other christinas. We$\ldots$ & &  muster up the courage to put down Braves fans. I$\ldots$\\\cline{2-2}\cline{4-4}
			& $\ldots$I've heard it said that the accounts we have   & & $\ldots$ NPR's Morning Edition aired a report this morning\\
			& of Christs life and ministry in the Gospels were$\ldots$ & &  to get (4/19) on Hispanic/Latin American players in MLB$\ldots$ \\\hline
			Atheism& $\ldots$This article attempts to provide a general  & Hockey & $\ldots$ Would Kevin Dineen play for the Miami Colons???   \\
			& introduction to atheism. Whilst I
			have tried to be$\ldots$ & & As a Flyers fan, I resent you making Kevin Dineen$\ldots$\\\cline{2-2}\cline{4-4}
			& $\ldots$Science is wonderful at answering most of our  & & $\ldots$Good point - there haven't even been any recent posts 
			\\
			& questions. I'm not the type
			to question scientific$\ldots$ & & about ULf! Secretly, I'm convinced that he is responsible $\ldots$\\\hline
		\end{tabular}}
\end{table}
%\begin{figure}
%	\centering
%	\begin{subfigure}[t]{0.3\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{clean_run_figures/lr_01_2_extended.pdf}
%		\caption{$m=2$}		
%	\end{subfigure}
%	\begin{subfigure}[t]{0.3\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{clean_run_figures/lr_01_20_extended.pdf}
%		\caption{$m=20$}		
%	\end{subfigure}
%	\begin{subfigure}[t]{0.3\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{clean_run_figures/lr_01_50_extended.pdf}
%		\caption{$m=50$}		
%	\end{subfigure}
%	\caption{Test error rates found by solving the camouflage framework. We also show random and oracle error for comparison. Error bars are also shown. Beam search and uniform sampling solvers were run for two additional hours than the NLP solver.}~\label{fig:lr_results_extended}
%\end{figure}




==> arxiv_Paper (copy)/conc.tex <==

We introduced the training set camouflage setting where a carefully constructed training set can be sent over an open channel with the intention of training a machine learner on a secret classification task.
Using this framework, an agent can hide the intention of the secret task from a third party observer.
We formulated training set camouflage as a bilevel optimization problem and provided methods to approximately solve it based on non-linear programming and combinatorial search.

We conducted empirical experiments on logistic regression and artificial neural network learners with real-world data to see if such a subterfuge is actually possible.
Our results suggest that it is indeed possible to approximately recover the classifier on the original task.
%Among the proposed solvers beam search performed the best overall and is applicable for a wide range of learners.
%Thus beam search should be the preferred solver for Alice.
Among the proposed solvers NLP performed the best overall.

%In some cases, we even get identical results that was found after training on the secret set as well. 
%The present paper should serve as a warning on the existence of such camouflage attacks.

In the future, we plan to devise defensive mechanisms to detect such subterfuge.
We also plan to explore training set camouflage in a cross modality domain (e.g., when the secret task is text classification while the camouflage task is image classification) and in settings where Alice does not have complete information about Eve or Bob.
We also intend to further investigate Alice's capability to remain undetected while altering Bob's learned model in a training-time attack setting, where Alice perturbs an already existing training set, rather than creating one.




==> arxiv_Paper (copy)/discussions.tex <==
We introduced the training set camouflage setting where a carefully constructed training set can be sent over an open channel with the intention of training a machine learner on a secret classification task.
Using this framework, an agent can hide the intention of the secret task from a third party observer.
Our experimental results show that training set camouflage is indeed a plausible threat.
We present three approaches to solve the optimization problem.
We observe that all three solvers perform well but both NLP and beam search outperform uniform sampling in all cases.
The NLP solver often performs a bit better than beam search.
This suggests that for the logistic regression learner NLP is Alice's preferred solver of choice.
However, the NLP solver cannot be applied to all possible learners (non-convexity prevents the application of KKT conditions).
Thus in such cases beam search becomes the preferred solver.


	
We note that $\mmd$ is stronger with larger sample sizes.
It will be harder for Alice to fool Eve given a large camouflage pool $C$ and also if she is forced to select a large camouflaged training set $D$. 
$\mmd$ is also stronger with smaller feature dimensions~\cite{gretton2012kernel}.
Also, it is harder for Alice to fool Eve if she increases the value of $\alpha$.
Since $\alpha$ is the upper bound of the probability of the Type I error for the null hypothesis i.e., the camouflage pool and camouflaged training set come from the same distribution, increasing $\alpha$ allows Eve to become more suspicious.
As future work we plan to devise defensive strategies against Alice.
In such scenarios it is advisable to assume that Eve's detection function is known to the attacker (Kerckhoffs's principle~\cite{kerckhoffs18831,kerckhoffs18832}) which we make here.
	
	
We note that camouflage seems easier for Alice to do if the cover task is in fact somewhat confusable, presumably because she can generate different decision boundaries by picking from overlapping camouflage items.
This can be imagined easily in the 2D case with two overlapping point clouds forming the cover task.
In such a scenario any separable secret task (no overlap between the secret task instances) can be taught to Bob by Alice. 
One interesting open question is whether there is a \textit{universal} cover task for all secret tasks. %(they must use the same feature representation, of course).
We also note that achieving Alice's goal becomes much harder in the multi-class setting as finding a cover task becomes more challenging.
	
As mentioned previously, Bob fixed his learning hyperparameters (e.g., regularization parameter of the logistic regression).
This was done for speed.
However, nothing prevents Bob from using cross validation~\cite{kohavi1995study}. 
Cross validation is popular technique used in machine learning where the learner is trained multiple times on different subsets of the whole training set to tune the hyperparameters of the learner.
Alice would simply emulate the same cross validation while optimizing the camouflaged training set.
This can be easily done in beam search and uniform sampling, at the cost of more computation.
Unfortunately significant modifications will be required for NLP.
	
Also, the loss function $\ell$ used by Alice and Bob is the same, as seen in the upper and lower optimization problems in~\eqref{eq:MMDConstraint}.
It is straightforward to allow different losses.  For example, Bob may learn with the logistic loss since it is a standard learner, while Alice uses 0-1 loss to directly optimize Bob's accuracy.
	
%Moreover, we note that the assumption of Eve's detection function being known to Alice can be relaxed as well. If Alice does not have access to said detection function then it is possible for her to generate a surrogate of that function by probing Eve with multiple datasets (while not training Bob). Once Alice is confident about the surrogate function, she can again apply the same techniques to generate the camouflaged training set. We leave out this discussion for future work.
	
We note that training set camouflage can be extended to cross modality correspondence, e.g., use an image camouflage pool while the secret classification task is to classify text articles. 
Alice and Bob can communicate via the private channel to establish the correspondance between images features and text features. 
Another possible way to extend the camouflage pool is to allow perturbed instances as well.


==> arxiv_Paper (copy)/exp.tex <==

We investigated the effectiveness of training set camouflage through empirical experiments on real world datasets. 
Our results show that camouflage works on a variety of image and text classification tasks: 
Bob can perform well on the secret task after training on the camouflaged training set,
and the camouflaged training set passes Eve's test undetected.

\textbf{Bob}.  We considered two different learning algorithms for Bob: logistic regression and artificial neural network (ANN)~\cite{karabatak2009expert}.
Both of these learners are popular and regularly used in practice. 
For the logistic regression learner, the weight of the regularization parameter was set to $1$. 
We present the specification and results for the ANN in Appendix B.

\textbf{Eve}.
For our experimental purposes we used Maximum Mean Discrepancy ({\mmd})~\cite{gretton2012kernel} as Eve's detection function.
{\mmd} is a widely used two-sample test~\cite{dziugaite2015training} but cannot be directly used in the camouflage framework.
\todo{you have to briefly say why.   also this directly contradicts with the first sentence "we used MMD"}
We introduce {\mmd} and Eve used it in Appendix A.
The level-$\alpha$ for this detection function was set to $0.05$ (i.e., 95\% confidence). 


\textbf{Alice}.
%For the ANN Bob, Alice only used beam search and uniform sampling (nonconvexity prevents application of KKT); while for logistic regression she used all three  solvers. 
Alice constructed camouflaged training sets of size $m=20$, $100$ and $500$.
For all secret tasks Alice was allotted separate budgets to identify a suitable camouflage task and then the camouflaged training set.
Alice used uniform sampling with a search budget of $80,000$ to identify a suitable camouflage pool.
This meant that Alice stopped the search after training the logistic regression learner $80,000$ times.
For simplicity we assume that during this phase $m$ was set to $20$ for all cases.
Alice had a further budget of $80,000$ to find a camouflaged training set for both beam search and uniform sampling.
For beam search, she performed five random restarts each with a budget of $16,000$ and then used the best found training set.
Here the size of the beam was $10$ and for each training set in the beam, $50$ randomly selected neighbors were evaluated during each iteration.
%For beam search, the search budget was set to $200,000$, then repeated five times with random restarts.
%This meant that Alice stopped the search for a camouflaged training set after training the learner $200,000$ times.
The NLP solver does not have a notion of budget and Alice must seed the solver with some initial dataset.
Thus it cannot be directly compared with the other two solvers.
Alice performed a separate experiment with only $m=20$.
In this case the initial dataset was set to be the output found by the beam search solver.
The loss $\ell$ was logistic loss and squared loss for logistic regression and ANN, respectively. 


\textbf{Evaluation metrics}.
As is standard to estimate general performance, we used a separate test set, generated from the same distribution as the secret set $D_S$ and not known to any agent, to evaluate Bob's generalization error when trained on Alice's camouflaged training set $D$.
We compare this to two quantities:
(``random'') when Bob is trained on a uniform sample of size $m$ from the cover data distribution, which we expect to perform poorly; and 
(``oracle'') when Bob is trained directly on Alice's secret set $D_S$, ignoring Eve's presence.
The oracle gives us an estimate on how much performance Bob is losing due to camouflage.


\subsection{Datasets}

%We performed eight camouflage experiments: WM71, WMOA, GP52, GPOA, CABH, CAIM, DRBH and DRIM as described below.
%The first two letters in the acronyms encode the secret task, and the last two the cover task.
%In both WM71 and WMOA the secret task was woman vs. man (CIFAR-100), the cover task was handwritten digits 7 vs. 1 (MNIST) and orange vs. apple (CIFAR-100), respectively. 
%In GP51 and GPOA the secret task was handgun vs. phone image classification (OpenImages~\cite{openimages}),
%the cover was 5 vs 1 and orange vs. apple, respective.
%In CABH and CAIM the secret task was text classification on christian vs atheism (20-newsgroups), the cover tasks were baseball vs hockey and pc vs mac, respectively.
%In DRBH and DRIM the secret task was text classification on Democratic vs. Republican , the cover tasks were baseball vs hockey and pc vs mac, again.
%For all datasets, the positive/negative examples of the sensitive set were mapped to the positive/negative examples of the camouflage pool.
%We do so because we assume that Alice is not allowed to modify instances in the camouflage pool.
%Since Eve also has access to the same camouflage pool, such modifications will be easy to detect for her.

%We performed experiments for four secret tasks: women vs. man (CIFAR-100) images (WM), handgun vs. phone (OpenImages~\cite{openimages}) images (GP), christian vs. atheism (20-newsgroups) articles (CA) and Democratic vs. Republican (All The News dataset~\cite{allthenews2017}) articles (DR).
We performed experiments for four secret tasks: WM (CIFAR-100~\cite{krizhevsky2009learning}), GP (OpenImages~\cite{openimages}), CA (20-newsgroups~\cite{joachims1996probabilistic}) and DR (All The News dataset~\cite{allthenews2017}).
The two letters in the acronym represent the two classes in the corresponding task.
The first two tasks were image classification while the remaining two were text classification.
For the image tasks we selected eight candidate cover tasks. 
Six of them were from the MNIST handwritten digits: 17, 71, 25, 52, 69 and 96.
The other two were from the CIFAR-100 dataset: OA and OA.
Similarly for the text tasks we also selected eight candidate cover tasks.
All of them were from the 20-newsgroups dataset: BS, HB, IM, MI, AM, MA, MX and XM.
As before the acronyms here represent the class names.


For images we used ResNet~\cite{he2016deep} to generate feature vectors of dimension $2048$. 
For text we used Word2Vec~\cite{mikolov2013efficient} to generate feature vectors of dimension $300$ by averaging over the word vectors in an article.
A summary of the sensitve sets and camouflage pools (along with the corresponding classes) can be found in Table~\ref{tab:dataSum}.

%\begin{table*}[!htb]
%	\centering
%	\caption{Dataset Summary}~\label{tab:dataSum}
%	\resizebox{\textwidth}{!}{%
%	\begin{tabular}{|l|l|r|r|r|r|r|r|r|}
%		\hline
%		\multicolumn{1}{|c|}{\textbf{Name}} & \multicolumn{1}{|c|}{\textbf{Type}} & \multicolumn{1}{|c|}{\textbf{\# Features}} & \multicolumn{1}{|c|}{\textbf{\# Camouflage }} & \multicolumn{1}{|c|}{\textbf{\# Camouflage }} & \multicolumn{1}{|c|}{\textbf{\# Secret }} & \multicolumn{1}{|c|}{\textbf{\# Secret }} & \multicolumn{1}{|c|}{\textbf{\# Test }} & \multicolumn{1}{|c|}{\textbf{\# Test }} \\
%		 &  &  & \multicolumn{1}{|c|}{\textbf{Pool Positive}} & \multicolumn{1}{|c|}{\textbf{Pool Negative}} & \multicolumn{1}{|c|}{\textbf{Positive}} & \multicolumn{1}{|c|}{\textbf{Negative}} & \multicolumn{1}{|c|}{\textbf{Positive}} & \multicolumn{1}{|c|}{\textbf{Negative}} \\
%		\hline
%		WM71 & Image & $2048$ & $600$ & $600$ & $500$ & $500$ & $100$ & $100$ \\\hline
%		WMOA & Image & $2048$ & $600$ & $600$ & $500$ & $500$ & $100$ & $100$ \\\hline
%		GP52 & Image & $2048$ & $600$ & $600$ & $400$ & $400$ & $100$ & $100$ \\\hline
%		GPOA & Image & $2048$ & $600$ & $600$ & $400$ & $400$ & $100$ & $100$ \\\hline
%		CABH & Text & $300$ & $994$ & $999$ & $599$ & $480$ & $398$ & $319$ \\\hline
%		CAIM & Text & $300$ & $982$ & $963$ & $599$ & $480$ & $398$ & $319$  \\\hline
%		DRBH & Text & $300$  & $994$  & $999$ & $800$ & $800$ & $200$ & $200$ \\\hline
%		DRIM & Text & $300$  & $982$ & $963$ & $800$ & $800$ & $200$ & $200$ \\\hline
%	\end{tabular}
%	}
%\end{table*}

%\begin{table*}[!htb]
%	\centering
%	\caption{Dataset Summary}~\label{tab:dataSum}
%	\resizebox{\textwidth}{!}{%
%		\begin{tabular}{|l|l|r|r|r|r|r|r|r|}
%			\hline
%			\multicolumn{1}{|c|}{\textbf{Name}} & \multicolumn{1}{|c|}{\textbf{Type}} & \multicolumn{1}{|c|}{\textbf{\# Features}} & \multicolumn{1}{|c|}{\textbf{\# Camouflage }} & \multicolumn{1}{|c|}{\textbf{\# Camouflage }} & \multicolumn{1}{|c|}{\textbf{\# Secret }} & \multicolumn{1}{|c|}{\textbf{\# Secret }} & \multicolumn{1}{|c|}{\textbf{\# Test }} & \multicolumn{1}{|c|}{\textbf{\# Test }} \\
%			&  &  & \multicolumn{1}{|c|}{\textbf{Pool Positive}} & \multicolumn{1}{|c|}{\textbf{Pool Negative}} & \multicolumn{1}{|c|}{\textbf{Positive}} & \multicolumn{1}{|c|}{\textbf{Negative}} & \multicolumn{1}{|c|}{\textbf{Positive}} & \multicolumn{1}{|c|}{\textbf{Negative}} \\
%			\hline
%			%WM71 & Image & $2048$ & $600$ & $600$ & $500$ & $500$ & $100$ & $100$ \\\hline
%			WMOA & Image & $2048$ & $600$ & $600$ & $500$ & $500$ & $100$ & $100$ \\\hline
%			GP96 & Image & $2048$ & $600$ & $600$ & $400$ & $400$ & $100$ & $100$ \\\hline
%			%GPOA & Image & $2048$ & $600$ & $600$ & $400$ & $400$ & $100$ & $100$ \\\hline
%			CABH & Text & $300$ & $994$ & $999$ & $599$ & $480$ & $398$ & $319$ \\\hline
%			%CAIM & Text & $300$ & $982$ & $963$ & $599$ & $480$ & $398$ & $319$  \\\hline
%			DRBH & Text & $300$  & $994$  & $999$ & $800$ & $800$ & $200$ & $200$ \\\hline
%			%DRIM & Text & $300$  & $982$ & $963$ & $800$ & $800$ & $200$ & $200$ \\\hline
%		\end{tabular}
%	}
%\end{table*}

\begin{table}
	\centering
	\caption{Summary of secret sets and camouflage pools.}~\label{tab:dataSum}
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		\textbf{Dataset} & \textbf{Type} & \textbf{\# Features} & \textbf{class 1} & \textbf{class 2} & \textbf{\# class 1} & \textbf{\# class 2} \\\hline
		WM & Image & 2048 & \textbf{w}oman & \textbf{m}an & 500 & 500 \\\hline
		GP & Image & 2048 & hand\textbf{g}un & \textbf{p}hone & 400 & 400 \\\hline
		CA & Text & 300 & \textbf{c}hristian & \textbf{a}theist & 599 & 480 \\\hline
		DR & Text & 300 & \textbf{d}emocratic & \textbf{r}epublican & 800 & 800 \\\hline
		17 & Image & 2048 & digit \textbf{1} & digit \textbf{7} & 600 & 600 \\\hline
		25 & Image & 2048 & digit \textbf{2} & digit \textbf{5} & 600 & 600 \\\hline
		69 & Image & 2048 & digit \textbf{6} & digit \textbf{8} & 600 & 600 \\\hline
		OA & Image & 2048 & \textbf{o}range & \textbf{a}pple & 600 & 600 \\\hline
		BH & Text & 300 & \textbf{b}aseball & \textbf{h}ockey & 994 & 999 \\\hline
		IM & Text & 300 & \textbf{i}bm & \textbf{m}ac & 982 & 963 \\\hline
		AM & Text & 300 & \textbf{a}utos & \textbf{m}otorcycles & 990 & 996 \\\hline
		MX & Text & 300 & \textbf{m}s-windows & windows \textbf{x} &985 & 988 \\\hline
	\end{tabular}
\end{table}


%The formation of the sensitive sets, camouflage pools and test sets are described as follows.
%In both the WM71 and WMOA datasets, the sensitive sets were comprised of images from the popular CIFAR-100 datasets. 
%The classification task was to differentiate between woman and man images. 
%%The training and test images of woman and man found in the CIFAR-100 dataset formed the sensitive set and test set respectively. 
%For the candidate pool of WM71, we used the popular MNIST dataset. 
%The only digits used were $7$ and $1$. 
%We sampled $600$ images at random to generate the camouflage pool. 
%For WMOA dataset, the camouflage pool was created by combining the orange and apple images from CIFAR-100. 
%OpenImages~\cite{openimages} is a well known dataset for image classification tasks. 
%For GP52 and GPOA, we selected $400$ images each at random from the classes Handgun and Mobile Phone to form the sensitive set. 
%A further $100$ images (no overlap with sensitive set) for each class were selected in a similar manner to form the test set. 
%The camouflage pool for GP52 was formed in the same manner as in WM71 except that the images used were $5$ and $2$. 
%The camouflage pool for GPOA was the same as for WMOA.
%
%20 Newsgroups is a popular text dataset. 
%The classification task for CABH and CAIM were to differentiate between articles with labels soc.religion.christian and alt.atheism. 
%The camouflage pool for CABH was created from articles with labels rec.sport.baseball and rec.sport.hockey. 
%Similarly, the camouflage pool for CAIM was created from articles with labels comp.sys.ibm.pc.hardware and comp.sys.mac.hardware.
%All the news is a text dataset~\cite{allthenews2017} that contains news articles from different sources like Breitbart, Washington Post, Fox News etc. 
%Some of these news articles are traditionally leaning towards the Grand Old Party (Republican) while others towards the Democratic Party. 
%In particular, we identified articles published in Breitbart and Fox News to be leaning towards Republicans while articles published in CNN and Washington Post were identified to be Democratic leaning. 
%We sampled $800$ such articles from each group to form the sensitive set for both DRBH and DRIM. 
%Further $200$ articles (no overlap with sensitive set) from each group were sampled to form the test set. 
%The camouflage pools were the same as in CABH and CAIM respectively. 	 

Alice first selected a suitable camouflage pool for each of the secret tasks.
For each candidate task she used a search budget of $10,000$ (allotted a total of $80,000$ budget).
The results of this phase are shown in Table~\ref{tab:imageCandSelect} and \ref{tab:textCandSelect}.
It can be seen that the camouflage pools selected for WM, GP, CA and BH are OA, 96, BH and BH respectively.
The top three camouflaged training sets for GP identified during this phase is shown in Figure~\ref{fig:candidateCover}.

\begin{table}[!htb]
	\centering
	\caption{Logistic loss ($\frac{1}{|D_S|}\sum_{(\tx,\ty)\in D_S}\log(1+\exp(-\ty w^\top\tx))$) after performing uniform sampling search with $m=20$ and search budget $10,000$ for image secret tasks. The best results for each secret task is shown in bold.}~\label{tab:imageCandSelect}
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
		\hline
		\backslashbox{Secret}{Camouflage}
		&\makebox[2em]{17}&\makebox[2em]{71}
		&\makebox[2em]{25}&\makebox[2em]{52} &\makebox[2em]{69}&\makebox[2em]{96}
		&\makebox[2em]{OA}&\makebox[2em]{AO}\\\hline 
		%& 17 & 71 & 25 & 52 & 69 & 96 & OA & AO \\\hline
		WM & $0.790$ & $0.611$ & $0.672$ & $0.688$ & $0.798$ & $0.679$ & $\mathbf{0.584}$ & $0.731$ \\\hline
		GP & $0.480$ & $0.510$ & $0.433$ & $0.390$ & $0.632$ & $\mathbf{0.337}$ & $0.510$ & $0.531$ \\\hline
	\end{tabular}
\end{table}

\begin{table}[!htb]
	\centering
	\caption{Logistic loss after performing uniform sampling search with $m=20$ and search budget $10,000$ for text secret tasks. The best results for each secret task is shown in bold.}~\label{tab:textCandSelect}
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
		\hline
		\backslashbox{Secret}{Camouflage}
		&\makebox[2em]{BH}&\makebox[2em]{HB}
		&\makebox[2em]{IM}&\makebox[2em]{MI} &\makebox[2em]{AM}&\makebox[2em]{MA}
		&\makebox[2em]{MX}&\makebox[2em]{XM}\\\hline 
		%& 17 & 71 & 25 & 52 & 69 & 96 & OA & AO \\\hline
		CA & $\mathbf{0.672}$ & $0.673$ & $0.676$ & $0.675$ & $0.676$ & $0.674$ & $0.675$ & $0.675$ \\\hline
		DR & $\mathbf{0.681}$ & $0.684$ & $0.682$ & $0.683$ & $0.682$ & $0.682$ & $0.682$ & $0.683$ \\\hline
	\end{tabular}
\end{table}

\begin{figure}[htb]
	\centering
	\begin{subfigure}[t]{0.8\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/openimages_sample.pdf}
		\caption{Samples from the secret task Gun vs. Phone (GP)}~\label{fig:GP}
	\end{subfigure}
	
	\begin{subfigure}[t]{0.8\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/GP96.pdf}
		\caption{Camouflaged training set using 9 vs. 6}~\label{fig:GP96}
	\end{subfigure}
	
	\begin{subfigure}[t]{0.8\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/GP52.pdf}
		\caption{Camouflaged training set using 5 vs 2}~\label{fig:GP52}
	\end{subfigure}
	\begin{subfigure}[t]{0.8\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/GP25.pdf}
		\caption{Camouflaged training set using 2 vs. 5}~\label{fig:GP25}
	\end{subfigure}
	\caption{Samples of GP secret set, and the top three camuflaged training set found during the candidate selection phase.}~\label{fig:candidateCover}
\end{figure}


%\begin{table}
%	\centering
%	\caption{Number of models trained per hour for logistic regression learner using Random Argmin search. Total number of models trained (on a $8$ core machine) for individual experiments is $10000$.}
%	\begin{tabular}{|c|c|c|}
%		\hline
%		Dataset & $100$ & $500$ \\\hline
%		WM17 & $243,063$ & $73,099$ \\\hline
%		CABH & $250,963$ & $158,469$  \\\hline
%	\end{tabular}
%\end{table}

%\begin{table}
%	\centering
%	\caption{Number of models trained per hour for ANN learner using Random Argmin search. Total number of models trained (on a $8$ core machine) for individual experiments is $10000$.}
%	\begin{tabular}{|c|c|c|c|}
%		\hline
%		Dataset & $20$ & $100$ & $500$ \\\hline
%		WM17 & $15,272$ & $12,939$ & $8,435$  \\\hline
%		CABH & $15,764$ & $15,223$ & $12,474$ \\\hline
%	\end{tabular}
%\end{table}

\subsection{Results}
We present our results for beam search and uniform sampling in Figure~\ref{fig:lr_results}.
%In this figure, we also show the random error and the oracle error as well for comparison.
%For brevity, we only show $\trainSize=20$ and $\trainSize=500$ results respectively for the image and text datasets.
%But we note that the results presented herein are representative of all experiments performed.
%For the image and text datasets we only show the results when $\trainSize=20$ and $\trainSize=500$ respectively for brevity.
%For the ANN we only used the beam search solver as the NLP solver is not applicable.
%This is because for this learner the NLP solver is not applicable.
%For brevity, we only show $\trainSize=20$ and $\trainSize=500$ results respectively for the image and text experiments.
%But we note that the results presented herein are representative of all experiments performed.
%Each of these figures show the results for one particular $m$ value (20, 100 or 500).
We observe that Alice, using either solver can find much better camouflage training sets than random and in many cases approach oracle.
Keep in mind that Alice's solutions do not trigger Eve's suspicion function.
This shows that such subterfuges are plausible in practice and can actually yield good results from Alice's point of view.


%We show the test error rate after Bob is trained on the sensitive set (baseline error) and also when Bob is trained on the camouflaged training set. Moreover, we also show the length of the training set along with value produced by Eve's detector function (always negative) for our solvers. Looking at the results it can be seen that the test error rate found by both NLP and beam search are relatively close to the baseline error. This is particularly true for the logistic regression learner (note that, for neural network learner we had a reduced search budget). 

%\begin{figure}[!htb]
%	\centering
%	\begin{subfigure}[t]{0.45\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{figures/lr_error_bars.pdf}
%		\caption{Logistic Regression Learner}
%	\end{subfigure}
%	\begin{subfigure}[t]{0.45\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{figures/nn_error_bars.pdf}
%		\caption{Artificial Neural Network Learner}		
%	\end{subfigure}
%	\caption{Test error rates found by solving the camouflage framework. We also show random (with error bars) and oracle error for comparison. For image and text datasets we show results for $\trainSize=20$ and $\trainSize=500$ respectively for brevity.}~\label{fig:results}
%\end{figure}

\begin{figure}[!htb]
	\centering
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/lr_error_bars_20.pdf}
		\caption{$m=20$}
	\end{subfigure}
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/lr_error_bars_100.pdf}
		\caption{$m=100$}
	\end{subfigure}
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/lr_error_bars_500.pdf}
		\caption{$m=500$}
	\end{subfigure}
	\caption{Test error rates found by solving the camouflage framework for the logistic regression learner using beam search and uniform sampling. We also show random (with error bars) and oracle error for comparison.}~\label{fig:lr_results}
\end{figure}




%\begin{table*}[!htb]
%	\centering
%	\caption{Test error rate found by solving the camouflage problem. For image and text datasets we show results of length $20$ and $500$ respectively }~\label{tab:results}
%	%\resizebox{\textwidth}{!}{%
%		\begin{tabular}{|l|r|r|r|r||r|r|r|}
%			\hline
%			\textbf{Name} & \multicolumn{4}{|c||}{\textbf{Bob=Logistic Regression}} & \multicolumn{3}{|c|}{\textbf{Bob=Neural Network}}\\\cline{2-8}	
%			& \multicolumn{1}{|c|}{\textbf{Baseline}} & \multicolumn{1}{|c|}{\textbf{NLP}}  & \multicolumn{1}{|c|}{\textbf{Beam Search}} & \textbf{Oracle} & \multicolumn{1}{|c|}{\textbf{Baseline}} & \multicolumn{1}{|c|}{\textbf{Beam Search}} & \textbf{Oracle} \\
%			& \multicolumn{1}{|c|}{\textbf{Error}} & \multicolumn{1}{|c|}{\textbf{Error}} & \multicolumn{1}{|c|}{\textbf{Error}}& \multicolumn{1}{|c||}{\textbf{Error}}& \multicolumn{1}{|c|}{\textbf{Error}}& \multicolumn{1}{|c|}{\textbf{Error}}& \multicolumn{1}{|c|}{\textbf{Error}}\\\hline
%			WM71 & $0.402 (0.009)$ & $0.335$ & $0.255$ & $0.185$ & $0.452 (0.018)$ & $0.280$ & $0.160$ \\\hline
%			WMOA & $0.426 (0.012)$ & $0.310$ & $0.265$ & $0.185$ & $0.460 (0.013)$ & $0.265$ & $0.160$ \\\hline
%			GP52 & $0.482 (0.031)$ & $0.065$ & $0.025$ & $0.030$ & $0.499 (0.015)$ & $0.115$ & $0.055$ \\\hline
%			GPOA & $0.488 (0.016)$ & $0.340$ & $0.045$ & $0.030$ & $0.528 (0.029)$ & $0.120$ & $0.055$ \\\hhline{|=|=|=|=|=||=|=|=|}
%			CABH & $0.454 (0.002)$ & $0.243$ & $0.255$ & $0.162$ & $0.450 (0.002)$ & $0.278$ & $0.144$ \\\hline
%			CAIM & $0.449 (0.002)$ & $0.240$ & $0.259$ & $0.162$ & $0.460 (0.010)$ & $0.339$ & $0.144$ \\\hline
%			DRBH & $0.497 (0.005)$ & $0.300$ & $0.273$ & $0.243$ & $0.473 (0.006)$ & $0.368$ & $0.248$ \\\hline
%			DRIM & $0.495 (0.006)$ & $0.298$ & $0.303$ & $0.243$ & $0.500 (0.006)$ & $0.353$ & $0.248$ \\\hline
%		\end{tabular}%}
%\end{table*}


%\begin{table*}[!htb]
%	\centering
%	\caption{Best test error rate found. We also show the corresponding length of the camouflaged training set and value of the detector function along with the baseline test error rate}
%	\resizebox{\textwidth}{!}{%
%	\begin{tabular}{|l|r|r|r|r|r|r|r||r|r|r|r|}
%		\hline
%		\textbf{Name} & \multicolumn{7}{|c||}{\textbf{Logistic Regression}} & \multicolumn{4}{|c|}{\textbf{Neural Network}}\\\cline{2-12}	
%		& \textbf{Baseline} & \multicolumn{3}{|c|}{\textbf{NLP}}  & \multicolumn{3}{|c||}{\textbf{Beam Search}} & \textbf{Baseline} & \multicolumn{3}{|c|}{\textbf{Beam Search}} \\\cline{3-8}\cline{10-12}
%		& \multicolumn{1}{|c|}{\textbf{Error}} & \multicolumn{1}{|c|}{\textbf{Error}} & \multicolumn{1}{|c|}{\textbf{Length}} & \multicolumn{1}{|c|}{$\suspicion(\optSeq)$} & \multicolumn{1}{|c|}{\textbf{Error}} & \multicolumn{1}{|c|}{\textbf{Length}} & \multicolumn{1}{|c||}{$\suspicion(\optSeq)$} & \multicolumn{1}{|c|}{\textbf{Error}} & \multicolumn{1}{|c|}{\textbf{Error}} & \multicolumn{1}{|c|}{\textbf{Length}}& \multicolumn{1}{|c|}{$\suspicion(\optSeq)$}\\\hline
%		WM71 & $0.185$ & $0.335$ & $20$ & $-0.815$ & $0.255$ & $20$ & $-0.910$ & $0.160$ & $0.280$ & $20$ & $-0.884$\\\hline
%		WMOA & $0.185$ & & & & $0.260$ & $100$ & $-0.427$ & $0.160$ & $0.265$ & $20$ & $-0.938$ \\\hline
%		GP52 & $0.030$ & & & & $0.030$ & $100$ & $-0.413$ & $0.055$ & $0.115$ & $20$ & $-0.885$ \\\hline
%		GPOA & $0.030$ & & & & $0.055$ & $100$ & $-0.330$ & $0.055$ & $0.120$ & $20$ & $-0.903$ \\\hline
%		CABH & $0.162$ & $0.243$ & $500$ & $-0.174$ & $0.255$ & $500$ & $-0.179$  & $0.144$ & $0.278$ & $500$ & $-0.227$\\\hline
%		CAIM & $0.162$ & $0.240$ & $500$ & $-0.177$ & $0.259$ & $500$ & $-0.176$ & $0.144$ & $0.339$ & $500$ & $-0.227$ \\\hline
%		DRBH & $0.243$ & $0.300$ & $500$ & $-0.130$ & $0.273$ & $500$ & $-0.123$ & $0.248$ & $0.335$ & $100$ & $-0.401$ \\\hline
%		DRIM& $0.243$ & $0.298$ & $500$ & $-0.156$ & $0.303$ & $500$ & $-0.145$ & $0.248$ & $0.323$ & $100$ & $-0.389$ \\\hline
%	\end{tabular}}
%\end{table*}



%\begin{table}[!htb]
%	\centering
%	\caption{Test error rate for neural network learner. We also show the corresponding length of the training set and value of the detector function along with the baseline test error rate}~\label{tab:nnResults}
%	\resizebox{0.48\textwidth}{!}{%
%	\begin{tabular}{|l|r|r|r|r|}
%		\hline
%		\textbf{Name} & \textbf{Baseline} & \multicolumn{3}{|c|}{\textbf{Beam Search}} \\\cline{3-5}
%		& \multicolumn{1}{|c|}{\textbf{Error}} & \multicolumn{1}{|c|}{\textbf{Error}} & \multicolumn{1}{|c|}{\textbf{Length}} & \multicolumn{1}{|c|}{$\suspicion(\optSeq)$} \\\hline
%		WM71 & $0.160$ & $0.280$ & $20$ & $-0.884$\\\hline
%		WMOA & $0.160$ & $0.265$ & $20$ & $-0.938$ \\\hline
%		GP52 & $0.055$ & $0.115$ & $20$ & $-0.885$ \\\hline
%		GPOA & $0.055$ & $0.120$ & $20$ & $-0.903$ \\\hline
%		CABH & $0.144$ & $0.278$ & $500$ & $-0.227$\\\hline
%		CAIM & $0.144$ & $0.339$ & $500$ & $-0.227$ \\\hline
%		DRBH & $0.248$ & $0.335$ & $100$ & $-0.401$ \\\hline
%		DRIM & $0.248$ & $0.323$ & $100$ & $-0.389$ \\\hline
%	\end{tabular}}
%\end{table}

%We show average Alice's loss with respect to search budget for the logistic regression learner in Figure~\ref{fig:manWomanBudget}. As expected, Alice's loss gradually decreases as the search proceeds. But the reduction of loss slowly decreases. This reduction depends on the size of the camouflaged training set. The larger the budget, the more important it is to increase the search budget. 

%\begin{figure}[!htb]
%	\centering
%	\includegraphics[width=0.45\textwidth]{figures/CIFAR-100_1_7_1_inhomo_logistic_200000_10_50_set_lr_best_val_errors2.pdf}
%	\caption{Search Budget vs Alice's Error for WM71 using different training sizes for logistic regression learner}~\label{fig:manWomanBudget}
%\end{figure}

%We show the camouflaged training sets (of size 20) found for the image classification tasks in Figure~\ref{fig:manWomanTraining}. We also show some samples of the sensitive set here as well. It can be seen that no relation can be seen between the camouflaged training sets and the sensitive dataset. Thus it is really hard for any eavesdropping agent to figure out the actual illicit classification task even when she suspects something malicious is going on. 


%\begin{figure*}[!tbh]
%	\centering
%	\includegraphics[width=0.95\textwidth]{figures/cifar_oa.pdf}
%\caption{Camouflaged training set using oranges vs. apples (WMOA). 
%The secret task woman vs. man was shown in Figure~\ref{fig:sd}, while another camouflage training set using 7 vs. 1 was shown in Figure~\ref{fig:cts}.
%}~\label{fig:moreexamples2}
%\end{figure*}




%Our experimental results show the feasibility of training set camouflage. 
%We observe that Alice, using either NLP, beam search solver or uniform sampling, can find much better camouflage training sets than random and in many cases approach oracle.
%Keep in mind that Alice's solutions do not trigger Eve's suspicion function.
%This shows that such subterfuges are plausible in practice and can actually yield good results from Alice's point of view.

\begin{table}[htb]
	\centering

	\caption{Camouflage results for the CABH experiment with $m=20$}
	\label{tab:CABH}

	\resizebox{\textwidth}{!}{%
		\begin{tabular}{|l|l|l|l|}
			\hline
			\multicolumn{2}{|c|}{\textbf{Sample of Secret Set}} & \multicolumn{2}{|c|}{\textbf{Sample of Camouflaged Training Set}} \\\hline
			\multicolumn{1}{|c|}{\textbf{Class}} & \multicolumn{1}{|c|}{\textbf{Article}} & \multicolumn{1}{|c|}{\textbf{Class}} & \multicolumn{1}{|c|}{\textbf{Article}} \\\hline
			Christianity & $\ldots$Christ that often causes christians to be very & Baseball & $\ldots$The Angels won their home opener against the\\ 
			&  critical of themselves and other christinas. We$\ldots$ & &  Brewers today before 33,000+ 
			at Anaheim Stadium$\ldots$\\\cline{2-2}\cline{4-4}
			& $\ldots$I've heard it said that the accounts we have   & & $\ldots$ interested in finding out how I might be able\\
			& of Christs life and ministry in the Gospels were$\ldots$ & &  to get two tickets for the All Star game in Baltimore$\ldots$ \\\hline
			Atheism& $\ldots$This article attempts to provide a general  & Hockey & $\ldots$ user and not necessarily those could anyone post   \\
			& introduction to atheism. Whilst I
			have tried to be$\ldots$ & & the game summary for the Sabres-Bruins game.$\ldots$\\\cline{2-2}\cline{4-4}
			& $\ldots$Science is wonderful at answering most of our  & & $\ldots$Tuesday, and the isles/caps game is going into 
			\\
			& questions. I'm not the type
			to question scientific$\ldots$ & & overtime. what does ESPN do. Tom Mees says, "we$\ldots$\\\hline
		\end{tabular}}
\end{table}
%		& $(231,038)$ & $(275,535)$ & - & - \\\hline
%		25 & $0.672$ & $0.433$ & - & - \\
%		& $(229,039)$ & $(284,157)$ & - & - \\\hline
%		52 & $0.688$ & $0.390$ & - & - \\
%		& $(223,429)$ & $(288,583)$ & - & - \\\hline
%		69 & $0.798$ & $0.632$ & - & - \\
%		& $(227,243)$ & $(280,036)$ & - & - \\\hline
%		96 & $0.679$ & $\mathbf{0.337}$ & - & - \\
%		& $(217,095)$ & $(275,772)$ & - & - \\\hline
%		OA & $\mathbf{0.584}$ & $0.510$ & - & - \\
%		& $(235,536)$ & $(278,660)$ & - & - \\\hline
%		AO & $0.731$ & $0.531$ & - & - \\
%		& $(233,628)$ & $(278,976)$ & - & - \\\hline
%		BH & - & - & $\mathbf{0.638}$ & $\mathbf{0.681}$ \\
%		& - & - & $(278,397)$ & $(203,911)$ \\\hline
%		HB & - & - & $0.673$ & $0.684$ \\
%		& - & - & $(290,539)$ & $(212,123)$ \\\hline
%		IM & - & - & $0.676$ & $0.682$ \\
%		& - & - & $(271,315)$ & $(321,232)$ \\\hline
%		MI & - & - & $0.675$ & $0.683$ \\
%		& - & - & $(277,706)$ & $(210,645)$ \\\hline
%		AM & - & - & $0.676$ & $0.682$  \\
%		& - & - & $(286,292)$ & $(345,258)$ \\\hline
%		MA & - & - & $0.674$ & $0.682$ \\
%		& - & - & $(303,565)$ & $(211,582)$ \\\hline
%		MX & - & - & $0.675$ & $0.682$  \\
%		& - & - & $(298,501)$ & $(211,204)$ \\\hline
%		XM & - & - & $0.675$  & $0.683$ \\
%		& - & - & $(288,489)$ & $(327,451)$ \\\hline
%	\end{tabular}
%\end{table}

Figures~\ref{fig:example} shows the results of WMOA when Bob's learner is logistic regression and the solver is beam search $(m=20)$.
Visually, the camouflaged training set $D$ bears no resemblance to the secret training set $D_S$.
This is true for text camouflage experiments as well, where articles in the camouflaged training sets have no obvious semantic connection to the sensitive task. 
See Table~\ref{tab:CABH} for results on the text experiment CABH.
This is indeed bad news for human Eves: not only did camouflage fooled MMD detector, it will also likely fool human inspectors.

%\subsubsection{NLP Results}
As mentioned previously, Alice ran a separate experiment for the NLP solver.
Alice evaluates a further $m$ training sets as part of the rounding procedure for NLP.
Let $I$ and $N$ identify the index vector of all instances in the initial dataset and all other instances in the camouflage pool respectively. 
Also let, $I'$ and $N'$ represent the sorted sequence of $I$ and $N$ such that $b_{I'_i} \ge b_{I'_i+1}$ and $b_{I'_i} \ge b_{I'_i+1}$. Now we define,
$T_c=[I'_1,I'_2,\ldots,I'_{m-c},N'_1,N'_2,\ldots,N'_c]$.  
Here $c\in\mathbb{Z}: c\in[0,m]$. 
Thus $T_0=I'$ and $T_m=[N'_1,N'_2,\ldots,N'_m]$.
Alice evaluates the training sets $\cand_{T_c}$ for all values of $c$. 
Note that she does not need to re-evaluate $T_0$. Thus the camouflaged training set found by using NLP solver is:
\begin{align}
\argmin_{c\in\mathbb{Z}: c\in[0,m]}& ~~&&\frac{1}{\vert \val \vert} \sum_{(\tx, \ty)\in \val}\tloss(\hat{\theta}, \tx, \ty)\nonumber\\
\text{s.t.}& ~~&&\hat{\theta} = \argmin_{\theta \in \Theta} \sum_{(\bfx, y)\in\cand_{T_c}} \closs(\theta, \bfx, y) + \frac{\lambda}{2} \Vert \theta \Vert^2\nonumber\\
& &&\suspicion(\cand,\cand_{T_c}) < 0
\end{align}
We compare this result against the other two solvers ran from the same amount of time (after the initial run with budget $80,000$). 
For WMOA, GP96, CABH and DRBH the NLP solver took $15886$, $49555$, $40$ and $65$ seconds respectively to finish on an Intel(R) Core(TM) i7-7700T CPU @2.90GHz machine. The results are shown in Figure~\ref{fig:nlp}.

%\begin{table}[!htb]
%	\centering
%	\caption{Time Required to Run NLP}
%	\begin{tabular}{|c|r|}
%		\hline
%		Dataset & Time (seconds)\\\hline
%		WMOA & 15886.38 \\\hline
%		GP96 & 49555.30 \\\hline
%		CABH & 39.52 \\\hline
%		DRBH & 65.33 \\\hline
%	\end{tabular}
%\end{table}

%\begin{table}[!htb]
%	\centering
%	\caption{NLP results for $m=20$ for Logistic Regression Learner. Improvements are highlighted in bold.}
%	\begin{tabular}{|c|c|c|c|}
%		\hline
%		\textbf{Dataset} & \textbf{Solver} & \textbf{Starting Test Error Rate} & \textbf{Final Test Error Rate} \\\hline
%		& NLP & 0.280 & 0.305  \\\cline{2-4}
%		WMOA & Beam Search & 0.280 & 0.300  \\\cline{2-4}
%		& Uniform Sampling & 0.340 & 0.325  \\\hline
%		& NLP & 0.075 & \textbf{0.070} \\\cline{2-4}
%		GP96 & Beam Search & 0.075 & \textbf{0.055} \\\cline{2-4}
%		& Uniform Sampling & 0.120 & 0.120 \\\hline
%		& NLP & 0.406 & 0.406 \\\cline{2-4}
%		CABH & Beam Search & 0.406 & 0.406 \\\cline{2-4}
%		& Uniform Sampling & 0.437 & 0.437 \\\hline
%		& NLP & 0.343 & \textbf{0.340} \\\cline{2-4}
%		DRBH & Beam Search & 0.343 & 0.343 \\\cline{2-4}
%		& Uniform Sampling & 0.375 & 0.375 \\\hline
%	\end{tabular}
%\end{table}

\begin{figure}[htb]
	\centering
	\centering
	\includegraphics[width=0.3\textwidth]{figures/nlp_lr_20.pdf}
	\caption{NLP results for $m=20$ for Logistic Regression Learner. Both beam search and uniform sampling solvers are run for the same amount of time as the NLP solver(after the initial $80,000$ budget). }~\label{fig:nlp}
\end{figure}


\subsection{Discussion}
Our experimental results show that training set camouflage is indeed a plausible threat.
We present three approaches to solve the optimization problem.
We observe that beam search largely outperforms uniform sampling.
%This suggests that our simple relaxation and rounding strategy in NLP needs improvement.
It should also be noted that the NLP solver can be used to slightly improve the solution of the input dataset.
%It should also be noted that the solutions found by NLP may not be feasible (i.e., $\suspicion(\cand,\optSeq)>0$).
%But this scenario did not occur during our experiments.
All these observations combined with the fact that beam search is also applicable to a wider range of learners (non-convexity prevents the application of KKT condition), makes beam search the preferred solver for Alice.

%\begin{figure}[htb]
%	\centering
%	\includegraphics[width=0.48\textwidth]{figures/diff_size_error_GP52.pdf}
%	\caption{Test error rate for different training set sizes. For both logistic regression and ANN we show the results for beam search on the GP52 dataset.}~\label{fig:diffSize}
%\end{figure}

%\begin{figure}[htb]
%	\centering
%	\includegraphics[width=0.48\textwidth]{figures/gen_error_lr_beam_search.pdf}
%	\caption{Secret set and Test set error rate for logistic regression using Beam Search. For image and text datasets we show results for $\trainSize=20$ and $\trainSize=500$ respectively for brevity.}~\label{fig:generalizationError}
%\end{figure}

We note that $\mmd$ is stronger with larger sample sizes.
It will be harder for Alice to fool Eve given a large camouflage pool $C$ and also if she is forced to select a large camouflaged training set $D$. 
$\mmd$ is also stronger with smaller feature dimensions~\cite{gretton2012kernel}.
Also, it is harder for Alice to fool Eve if she increases the value of $\alpha$.
Since $\alpha$ is the upper bound of the probability of the Type I error for the null hypothesis i.e., the camouflage pool and camouflaged training set come from the same distribution, increasing $\alpha$ allows Eve to become more suspicious.
Moreover, it is also possible for Eve to use other detection functions. 
The application of training set camouflage framework will remain the same regardless. 


%We designed the experiments so that Alice needs to teach the same secret task (e.g. woman vs. man) to Bob using two different cover tasks (e.g. 7 vs 1, and orange vs. apple).
%Interestingly, which cover task was used does not matter much.
%Conversely, Alice also needs to teach different secret tasks (e.g. woman vs. man, and gun vs. phone) to Bob using the same cover task (e.g. orange vs. apple). Alice also succeeds in this task to some degree.
We note that camouflage seems easier for Alice to do if the cover task is in fact somewhat confusable, presumably because she can generate different decision boundaries by picking from overlapping camouflage items.
This can be imagined easily in the 2D case with two overlapping point clouds forming the cover task.
In such a scenario any separable secret task (no overlap between the secret task instances) can be taught to Bob by Alice. 
One interesting open question is whether there is a \textit{universal} cover task for all secret tasks (they must use the same feature representation, of course).

As mentioned previously, Bob fixed his learning hyperparameters (e.g., regularization parameter of the logistic regression).
This was done for speed.
However, nothing prevents Bob from using cross validation~\cite{kohavi1995study}. 
Cross validation is popular technique used in machine learning where the learner is trained multiple times on different subsets of the whole training set to tune the hyperparameters of the learner.
Alice would simply emulate the same cross validation while optimizing the camouflaged training set.
This can be easily done in beam search and uniform sampling, at the cost of more computation.
This also suggests that these two solvers are much useful in practice than NLP.

Also, the loss function $\ell$ used by Alice and Bob is the same, as seen in the upper and lower optimization problems in~\eqref{eq:MMDConstraint}.
It is straightforward to allow different losses.  For example, Bob may learn with the logistic loss since it is a standard learner, while Alice may use 0-1 loss to directly optimize Bob's accuracy.

%Moreover, we note that the assumption of Eve's detection function being known to Alice can be relaxed as well. If Alice does not have access to said detection function then it is possible for her to generate a surrogate of that function by probing Eve with multiple datasets (while not training Bob). Once Alice is confident about the surrogate function, she can again apply the same techniques to generate the camouflaged training set. We leave out this discussion for future work.

It should also be noted that the training set camouflage can also be extended to cross modality correspondence, e.g., use an image camouflage pool with feature vectors of size $2048$ while the secret classification task is to classify text articles. 
In such a case Alice and Bob can decide beforehand to use the $2048$ most frequent words in the text articles to form bag of word (BOW) feature vectors for the secret classification task.


==> arxiv_Paper (copy)/framework.tex <==
In this section we describe the three agents Bob, Alice and Eve,  
and formulate a camouflage optimization problem for Alice, parametrized by Bob and Eve's definitions.


%\subsection{Bob}

The agent Bob uses a standard learning algorithm $\learner: \candset\mapsto\hypospace$ which, given a training set $D$, learns a hypothesis \(\learner(D)\) in a hypothesis space \(\hypospace\).
The resulting hypothesis maps instances in the input space \X to the output space \Y.
This can be multi-class classification (three or more classes) or regression, though in the present work we focus on binary classification.
We assume that Bob's learning algorithm is ``open source''.
That is, all information about $\learner$ is known to all agents.
However, Bob and Alice have shared knowledge on class naming: which class is positive and which negative.  
For $K$-class classification this shared knowledge requires $O(K\log K)$ bits, as Alice must communicate a mapping from \(K\) classes to \(K\) classes.
For example, when Alice sends Bob orange and apple images for the secret task of woman vs man, Alice must communicate to Bob whether orange maps to woman and apple to man, or vice versa.

%\subsection{Alice}

%Alice is the attacker.
Alice is an agent who wants to train Bob.
She has a secret classification task and the corresponding private dataset \(\val\).
In addition, she has access to a public pool of \(\candSize\) instances \(\cand=\{(\bfx_i, y_i)_{1:\candSize}\}\) (the {\em camouflage pool}) drawn i.i.d. from \(\mathbb{\cdist}_{(\bfx, y)}\) which we call the {\em cover data distribution}.
Note that this is not the  distribution from which \(\val\) is drawn.
In the preceding example, \(\mathbb{\cdist}_{(\bfx, y)}\) is the distribution over orange and apple images, whereas \(\val\) is a collection of photographs of women and men.


%\tikzmath{
%	\textVertDist=0.3;\rectHDist=3;\agentWidth=1.5;\agentHeight=0.8;
%	% coordinates for Eve
%	\eves1=0; \eves2=0; \evef1=\eves1+\agentWidth; \evef2=\eves2+\agentHeight;
%	\eveText1=(\eves1+\evef1)/2;\eveText2=\eves2-\textVertDist;
%	% coordinates for Bob
%	\bobs1=\evef1+\rectHDist; \bobs2=\eves2; \bobf1=\bobs1+\agentWidth; \bobf2=\evef2;
%	\bobText1=(\bobs1+\bobf1)/2;\bobText2=\bobs2-\textVertDist;
%	\bobHCenter=(\bobs1+\bobf1)/2;
%	%channel center
%	\channelCenter=(\eves2+\evef2)/2;
%	%selected instances
%	\sf1=\eves1-\rectHDist;\ss1=\sf1-2.5; \ss2=\eves2-1.4; \sf2=\evef2+2;
%	\slc=(\sf1+\ss1)/2;
%	\selectTextY1=\sf2+\textVertDist+0.5;\selectTextY2=\sf2+\textVertDist;
%	% coordinates for Alice
%	\alicef1=\ss1-1;\alices1=\alicef1-\agentWidth;\alices2=\eves2;\alicef2=\evef2;
%	%secret task
%	\secretHeight=2.5; \secretGap=0.75; \secrets1=\alices1-\secretGap;\secrets2=\alicef2+0.2;\secretf1=\alicef1+\secretGap;\secretf2=\secrets2+\secretHeight;
%	\secretHCenter=(\secrets1+\secretf1)/2;\sTaskY=\secretf2-\textVertDist;
%	% Database
%	\databaseY=5.8; \databaseTextX=\slc+2.7;
%	%plot
%	\plotLength=5;\plotX1=\bobs1-2;\plotY1=\bobf2+2+0.5;
%	%TODO:vsY, images
%}
%\begin{figure*}
%	\resizebox{0.7\textwidth}{!}{
%		\begin{tikzpicture}
%		\tikzstyle{l} = [draw, -latex',very thick];
%		\draw (\eves1,\eves2) rectangle (\evef1,\evef2) node[pos=0.5] (h2) {\textbf{\textcolor{red}{Eve:}} $\Psi$};
%		\node at (\eveText1,\eveText2) {Public Channel};
%		
%		\draw (\bobs1,\bobs2) rectangle (\bobf1,\bobf2) node[pos=0.5] (h3) {\textbf{\textcolor{red}{Bob}}};
%		\node at (\bobText1,\bobText2) {Learner $\mathcal{A}$};
%		%arrow from Eve to Bob
%		\path [l] (\evef1, \channelCenter) -- (\bobs1, \channelCenter);
%		
%		%Text box for learner training
%		\node(learning) at (\bobHCenter,\bobf2+2) {$\mathcal{A}(D)$};
%		\path[l] (\bobHCenter,\bobf2) -- (learning);
%		
%		%selected instances
%		\draw (\ss1,\ss2) rectangle (\sf1,\sf2);
%		\draw (\slc,\ss2) -- (\slc,\sf2);
%		\draw[very thick] (\sf1,\channelCenter) -- (\eves1,\channelCenter);
%		\node(select) at (\slc, \selectTextY1) {Select};
%		\path[l] (\slc,4.7) -- (select);
%		\node at (\slc, \selectTextY2) {Traning Set $D$};
%		%\node at (\slc+2.2, \selectTextY1-0.9) {Traning Set $D$};
%		%Database
%		\node (database) at (\slc,\databaseY) [cylinder, shape border rotate=90, draw,minimum height=2.8cm,minimum width=2.4cm,fill=white]
%		{\textcolor{white}{A}};
%		\node at (\databaseTextX,\databaseY) {Camouflage Pool $\mathcal{C}$};
%		
%		
%		%Alice
%		\draw (\alices1,\alices2) rectangle (\alicef1,\alicef2) node[pos=0.5] (h3) {\textbf{\textcolor{red}{Alice}}};
%		%Secret Task
%		\draw (\secrets1,\secrets2) rectangle (\secretf1,\secretf2);
%		\node at (\secretHCenter,\sTaskY) {Secret Task $D_S$};
%		
%		%Plot
%		\path[l] (\plotX1,\plotY1) -- (\plotX1+\plotLength,\plotY1);
%		\path[l] (\plotX1,\plotY1) -- (\plotX1,\plotY1+\plotLength);
%		\draw (\plotX1,\plotY1) -- (\plotX1+\plotLength-0.4,\plotY1+\plotLength-0.4);
%		
%		%Images
%		% Separation images
%		% Women
%		\node[inner sep=0pt] (w2) at (3.2,7.6) {\includegraphics[width=0.09\textwidth]{figures/w2.png}};
%		\node[inner sep=0pt] (w2) at (4.8,7.5) {\includegraphics[width=0.09\textwidth]{figures/w3.png}};
%		\node[inner sep=0pt] (w2) at (3.1,6.3) {\includegraphics[width=0.09\textwidth]{figures/w4.png}};
%		\node[inner sep=0pt] (w2) at (4.3,6.2)
%		{\includegraphics[width=0.09\textwidth]{figures/w5.png}};
%		\node[inner sep=0pt] (w2) at (3.2,5.1) {\includegraphics[width=0.09\textwidth]{figures/w6.png}};
%		% Men
%		\node[inner sep=0pt] (w2) at (6.95,6.6) {\includegraphics[width=0.09\textwidth]{figures/m2.png}};
%		\node[inner sep=0pt] (w2) at (5.8,5.4) {\includegraphics[width=0.09\textwidth]{figures/m3.png}};
%		\node[inner sep=0pt] (w2) at (4.35,4) {\includegraphics[width=0.09\textwidth]{figures/m4.png}};
%		\node[inner sep=0pt] (w2) at (5.5,4.15) {\includegraphics[width=0.09\textwidth]{figures/m5.png}};
%		\node[inner sep=0pt] (w2) at (6.8,4.25) {\includegraphics[width=0.09\textwidth]{figures/m6.png}};
%		% Secret Task Images
%		\node[inner sep=0pt] (w2) at (\secretHCenter+0.9,\sTaskY-1.2) {\includegraphics[width=0.09\textwidth]{figures/m1.png}};
%		\node[inner sep=0pt] (w2) at (\secretHCenter-0.9,\sTaskY-1.2) {\includegraphics[width=0.09\textwidth]{figures/w1.png}};
%		\node at (\secretHCenter,\sTaskY-1.2) {vs};
%		% Selected Instances Images
%		\node[inner sep=0pt] (w2) at (\ss1+0.65,\sf2-0.6) {\includegraphics[width=0.085\textwidth]{figures/7_1.png}};
%		\node[inner sep=0pt] (w2) at (\ss1+0.65,\sf2-1.7) {\includegraphics[width=0.085\textwidth]{figures/7_2.png}};
%		\node[inner sep=0pt] (w2) at (\ss1+0.65,\sf2-2.8) {\includegraphics[width=0.085\textwidth]{figures/7_3.png}};
%		\node at (\ss1+0.65,\sf2-3.65) {$\mathbf{\vdots}$};
%		\node[inner sep=0pt] (w2) at (\sf1-0.65,\sf2-0.6) {\includegraphics[width=0.085\textwidth]{figures/1_1.png}};
%		\node[inner sep=0pt] (w2) at (\sf1-0.65,\sf2-1.7) {\includegraphics[width=0.085\textwidth]{figures/1_2.png}};
%		\node[inner sep=0pt] (w2) at (\sf1-0.65,\sf2-2.8) {\includegraphics[width=0.085\textwidth]{figures/1_3.png}};
%		\node at (\sf1-0.65,\sf2-3.65) {$\mathbf{\vdots}$};
%		%Database Images
%		\node[inner sep=0pt] (w2) at (\ss1+0.65,\databaseY) {\includegraphics[width=0.085\textwidth]{figures/7_1.png}};
%		\node[inner sep=0pt] (w2) at (\sf1-0.65,\databaseY) {\includegraphics[width=0.085\textwidth]{figures/1_3.png}};
%		
%		\end{tikzpicture}}
%\end{figure*}


Alice seeks to select a camouflaged training set $D \subset \cand$ which she will send to Bob for training. 
Alice wants Bob to succeed on the secret task, thus she seeks to find a \(D\) which minimizes the risk of Bob's resulting model: 
\begin{align*}
\mathcal{L}_\learner(D) = \frac{1}{|\val|}\sum_{(\tx, \ty)\in \val}\tloss(\learner(D)(\tx), \ty)
\end{align*}
where \(\tloss(\hat y, y)\) is a loss function.
%where \(\tloss(\hat y, y)\) denotes a loss function for Bob predicting \(\hat y\) on an instance with true label \(y\). 
Note the private $D_S$ is used to define the quality of $D$.
Also, we note that $D_S$ and $D$ are in different domains.

%Note that we restrict Alice by requiring that \(D\) is a proper set (a subset of \(\cand\), not a multiset).
%In addition to computational and notation ease, this restriction is inspired by the following observation.
%Alice is going to send a training set to Bob which may be observed by the suspicious eavesdropper Eve.
%In practical settings, exact duplicates in a training set may appear suspect.
%We discuss relaxing this restriction in a later section \todo{we should do that}.



%\subsection{Eve}

Eve is a passive eavesdropper.
She observes the dataset $D$ which Alice sends to Bob, but does not alter it.
Her goal is to determine if $D$ is normal or suspicious.
Specifically, Eve is suspicious of any data unless it appears to be an i.i.d. sample drawn from  \(\mathbb{\cdist}_{(\bfx, y)}\).
She has access to the camouflage pool \(\cand\), but like Alice she cannot draw additional instances from \(\mathbb{\cdist}_{(\bfx, y)}\).
Eve uses \(\cand\) and a detection function $\suspicion:\candset\times\candset\mapsto\mathbb{R}_+$ to examine \(D\).
Here $\candset$ is the domain of all possible training sets.
She flags \(D\) as suspicious if \( \suspicion(\cand, D)\ge0 \).
It is useful to think of $\suspicion$ as a two-sample statistical test that aims to determine whether $\cand, D$ come from the same underlying distribution.
We envision Alice as Eve's adversary.
As with Bob, we assume that Eve is ``open source''.
Namely, Alice can see Eve's detection function $\suspicion$.


%\todo{Example to clarify Eve's role}


%\subsection{Alice's Optimization Problem}

The agents Alice and Eve have conflicting goals.
Alice aims to secretly communicate to Bob by way of constructing a training set, while Eve is suspicious and will flag any data sent to Bob if it looks suspect.
Bob dutifully learns a model and for our purposes has no explicit intentions.
We make explicit each Agent's knowledge in Table~\ref{tab:agentInfo}.
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\begin{table*}[htb]
	\centering
	\renewcommand{\tabcolsep}{1pt}
	\caption{Information available to different agents}~\label{tab:agentInfo}
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{|c|P{2.0cm}|P{2.0cm}|P{2.0cm}|P{2.0cm}|P{2.5cm}|}
			\hline
			
			\textbf{Agent} & \textbf{Secret Set} & \textbf{Camouflage Pool} & \textbf{Bob's Learner} & \textbf{Detection Function} & \textbf{Camouflaged Training Set}  \\
			& $\val$ & $\cand$ & $\learner$ & $\suspicion$ &  $\optSeq$\\\hline
			Bob & No & Yes/No & Yes & Yes/No & Yes \\\hline
			Alice & Yes & Yes & Yes & Yes & Yes \\\hline
			Eve & No & Yes & Yes & Yes & Yes \\\hline
		\end{tabular}
	}
\end{table*}

With the agents defined, we can now formulate Alice's goal:
\begin{align}
\argmin_{D\subset \cand} &  \frac{1}{|\val|}\sum_{(\tx, \ty)\in \val}\tloss(\learner(D)(\tx), \ty)\nonumber\\ 
\text{ s.t.
} & \suspicion(\cand, D)<0 
\label{aliceopti}
\end{align}
That is, she seeks a camouflaged training set \(D\) from the cover data pool.
$D$ should not be flagged as suspicious by Eve.
$D$ should also make Bob learn well, similar to as if Alice directly gave Bob her private data set \(\val\).
An example of the training set camouflage in action is shown in Figure~\ref{fig:framework}.
\begin{figure}[!htb]
	\centering
		%\includegraphics[width=\textwidth]{figures/IntroImage5.png}
		\includegraphics[width=0.9\textwidth]{clean_run_figures/IntroImage6.png}
	\caption{Training set camouflage framework. We show the three agents along with the classification task, camouflage pool, camouflage training set and Eve's detection function}~\label{fig:framework}
\end{figure}





==> arxiv_Paper (copy)/intro.tex <==

%Machine learning is a field of computer science that involves training a computer system (\textit{learner}) to learn from data (\textit{training set}) using statistical techniques.
%This field has received a lot of attention lately due to vast impacts in various applications ranging from disease detection~\cite{karabatak2009expert} to autonomous driving~\cite{chen2015deepdriving}.
%The \textit{tasks} that can be trained to a learner are broadly categorized into two groups.
%The first one is known as \textit{regression}, where given a data point (known as \textit{instance} in machine learning) the learner needs to predict a continuous output variable, e.g., given the credentials of a job candidate predict her salary.
%The second one is called \textit{classification} where the goal is to predict the value of discrete variable (\textit{class}) given an input instance, e.g., classify cat and dog images.
%In both cases the learner is first presented with a training set with corresponding the corresponding class values for each instance (\textit{label}) to make inferences from (also known as learning a \textit{model} or \textit{hypothesis}).
%In what follows we use the terms model and hypothesis interchangeably.


\begin{figure*}[h]
	\centering
	\begin{subfigure}[t]{0.9\textwidth}
		\centering
		%\includegraphics[width=\textwidth]{figures/WMOA.png}
		\includegraphics[width=\textwidth]{clean_run_figures/WMOA_NLP_training_set.pdf}
		\caption{Camouflaged training set}~\label{fig:cts}
	\end{subfigure}
	
	\begin{subfigure}[t]{0.9\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/CIFAR-100_Woman_Man_7_1_classified_sample_1238_resize.png}
		\caption{Secret classification task}~\label{fig:sd}
	\end{subfigure}
	\caption{Example of training set camouflage}~\label{fig:example}
\end{figure*}
Look at the classification training set shown in Figure~\ref{fig:cts}.
The top row contains instances of class positive (+), and the bottom shows instances of class negative (-).
These images can be fed into a machine learner to learn a model which will successfully classify future, previously unseen instances (images) as + or -.
If you think that the task is fruit image classification (orange vs. apples) then you have already been successfully fooled, in a sense to be made precise below.
The actual intended task is to classify woman vs. man, with samples shown in Figure~\ref{fig:sd}.
Indeed, a standard logistic regression learner~\cite{hosmer2013applied} trained on only the images in Figure~\ref{fig:cts} achieves high gender classification accuracy on the images in Figure~\ref{fig:sd}.

In this paper, we consider an agent Alice who has a secret classification task (e.g., classifying images of women and men) and a corresponding private training set (women and men images).
Alice wants to train a second agent, Bob, on the secret task.
However, the communication channel between them has an eavesdropper we refer to as a third agent Eve.
Eve takes the role of a data verifier, who will terminate communication (and refuse to deliver the data to Bob) if she is suspicious of what Alice is sending.
Sending the private training set would reveal Alice's intention; sending the model parameters directly will also raise suspicion.
Alice must camouflage the communication for it to look mundane to Eve, while avoiding excessive coding tricks with Bob beforehand.
In the present work, we show how Alice can construct a camouflaged training set on a {\em cover task}  which (i) does not look suspicious to Eve, and (ii) results in Bob learning an accurate model for the secret task. 
In the previous example, Eve noticed that Alice sent images of apples and oranges which seems benign, and knew nothing of Alice's secret task of women vs men.

%In the example of Figure~\ref{fig:example}, man vs woman image classification (from CIFAR-100~\cite{krizhevsky2009learning}) is the sensitive task, and hand-written digit recognition (1 vs 7 from the MNIST dataset~\cite{lecun1998mnist}) is the cover task.
%We call this setup \textit{training set camouflage}. % and make explicit the information available to each agent in Table~\ref{tab:agentInfo}.
%In this paper, we develop this framework and show that such a subterfuge is indeed possible.

%In particular, we consider the setting where a teacher, agent Alice wants to train a learner, agent Bob on a specific \textit{sensitive set}.
%A passive eavesdropper, agent Eve can view the training set Alice sends to Bob.
%Alice does not want Eve to get hold of the sensitive set or learn about the illicit classification task.
%To fool Eve, Alice instead sends Bob a training set whose instances are drawn from a separate pool (\textit{camouflage pool}).
%Alice's goal is two fold: (i) Alice does not want Eve to realize that Bob is actually being trained on the illicit classification task.
%(ii) After training, the risk of Bob's learned model must be minimized over the sensitive set.
%Figure~\ref{fig:intro} shows such an example.



%\begin{figure*}
%	\centering
%	\includegraphics[width=0.8\textwidth]{figures/IntroImage3.png}
%	\caption{Data Camouflage in Action}~\label{fig:intro}
%\end{figure*}



Hiding information in plain sight such that its presence is not suspected is known as steganography.
Steganography is not new. 
In the fifth century BCE  messengers would have their heads shaved and a message written on their scalp.
Regrowing their hair served to hide the message which would only be revealed because the intended recipient knew to shave the messenger's head~\cite{krenn2004steganography}.
In more modern times, steganographic techniques are used to detect unauthorized distribution of digital media~\cite{cox2005information}.

Note that, steganography is different from crypotgraphy~\cite{katz1996handbook,van2014encyclopedia}, where the goal is to hide the data content. 
In cryptography, the communicating agents have access to some particular key (pairs) which is used to encrypt and decrypt data. 
Cryptography cannot be used if someone monitoring the data can alter the data or stop the data transmission entirely. 
In such cases, steganography becomes important because we do not want any intervening eavesdropper to become suspicious and stop the data transmission.




The role and capabilities of the eavesdropper are key in selecting how to hide information.
Eve can be either passive and merely observes traffic~\cite{cachin1998information}, or active and tries to modify the hidden message~\cite{queirolo2011steganography,chandramouli2002mathematical}.
In this manuscript we assume a passive observer, whose only ability is to refuse to deliver Alice's message. 
To our knowledge, steganography for machine learning in this context is new.
In the area of adversarial learning~\cite{biggio2017wild}, however, much work has been done investigating how an agent can assert control over a learner by manipulating input data.
We note that training set camouflage differs from so called training-time or ``poisoning attacks"~\cite{kloft2010online} in two primary ways: (i) Alice aims to communicate information to Bob about a potentially completely unrelated task, not affect his behavior on the original task and (ii) Alice specifically aims to avoid detection by Eve.


%While developing a procedure of hiding information, the role and capabilities of the eavesdropper become key.
%%In a generic steganographic setting, the eavesdropper is known as the attacker which is different from the terminology we use (Alice is the attacker in our scenario).
%The analysis of data, by the eavesdropper Eve, to find the existence of hidden data is known as steganalysis.

%We note that attacking a machine learning algorithm is not new.
%One such branch of attack is known as "poisoning attacks"~\cite{kloft2010online} where the goal is to compromise the learner by injecting carefully designed instances into either the training or test set.
%One example would be the spam detection learners used by mail clients.
%Such learners use crowdsourced data to train.
%A malicious attacker can create thousands of fake mail accounts, and then mark a spam mail as "not spam" from all of the accounts in an attempt to fool the learner.
%The training set camouflage differs from such poisoning attacks in two primary ways: (i) Alice aims to communicate information to Bob about a potentially completely unrelated task, not affect his behavior on the original task and (ii) Alice specifically aims to avoid detection by Eve.


Due to the widespread use of machine learning in sensitive fields ranging from social media to health care, the study of the security ramifications of using ML techniques is well studied \cite{barreno2010security,lowd2005adversarial}.
The work presented herein adds to this conversation, as we reveal an additional avenue of attack. 
For example, Bob might be a model that classifies job applicants as ``should hire" and ``shouldn't hire".
The company may have many records (collected over years) of job applicants and how they performed.
It is expected from Alice to select a subset of these records and present to Bob, with the idea that training on the complete set is too time consuming.
But Alice may be a malicious agent and wants Bob to actually learn some additional bias (e.g., racial, gender etc.).
In such a scenario, Alice will select a subset of records that satisfies her goals while Eve's responsibility is to verify the data sent by Alice to Bob.
Our specific contributions in this paper are as follows: (i) We propose a general mathematical framework for defining how Alice can achieve training set camouflage.
(ii) We formulate a nonlinear-program based approach for performing Alice's task for a general class of learner (Bob) and eavesdropper (Eve), and two combinatorial-search based approaches for arbitrary learners/eavesdroppers.



%Its application dates back to ancient times from when Xerxes's ill intentions towards Greece was discovered to the more recent watermarking of digital content to detect unauthorized distribution~\cite{krenn2004steganography,cox2005information}.
 %In such a setting, the role of eavesdropper is very important.
 %She can be either passive and merely observes traffic~\cite{cachin1998information}, or active and try to modify the hidden message~\cite{queirolo2011steganography,chandramouli2002mathematical}.
% We extend this notion to machine learning where the goal is to train a learner in plain sight while hiding the true purpose.
% To the best of our knowledge such a setting has not be studied before.


==> arxiv_Paper (copy)/mmd.tex <==
One critical component of our camouflage framework is Eve's detection function \(\suspicion\) ---  how she determines if a training set is suspicious or not.
Eve's detection function is a two-sample test as its goal is to discern if the two sets $\cand, D$ are drawn from the same distribution or not.
In what follows we discuss using Maximum Mean Discrepancy ({\mmd})~\cite{gretton2012kernel} as Eve's detection function, as we do in our experiments.
{\mmd} is a widely used two-sample test~\cite{dziugaite2015training}, but, of course other detection functions can be used in~(\(\ref{aliceopti}\)).

We first review basic $\mmd$ following~\cite{gretton2012kernel}.
Let $p$ and $p'$ be two Borel probability measures defined on a topological space $\mathcal{Z}$.
Given a class of functions $\fspace$ such that $f:\mathcal{Z}\mapsto\R, f\in\fspace$, $\mmd$ is defined as 
\begin{equation}
	\mmd(p,p')=\sup_{f\in\fspace}(E_\bfz[f(\bfz)]-E_{\bfz'}[f(\bfz')])
%\label{eqn:mmd}
\end{equation}
Any unit ball in a reproducing kernel Hilbert space (RKHS) can be used as the function class $\fspace$ if the kernel is universal (e.g., Gaussian and Laplace kernels~\cite{steinwart2001influence}).
Using this function space, $\mmd$ is a metric.
This means $\mmd(p,p') = 0 \Leftrightarrow p = p'$.

Computing $\mmd$ requires the expectations to be known, which generally, is not the case in practice.
We obtain an empirical estimation by replacing the population expectations with empirical mean computed on 
i.i.d. samples $Z=\{\bfz_1,\ldots,\bfz_\candSize\}$ and $Z'=\{\bfz'_1,\ldots,\bfz'_\trainSize\}$ from $p$ and $p'$, respectively. 
%\begin{equation}
%	\mmd(Z,Z')=\sup_{f\in\fspace}\left(\frac{1}{m}\sum_{i=1}^mf(\bfz_i)-\frac{1}{n}\sum_{i=1}^nf(\bfz'_i)\right)
%\end{equation}
We define
\begin{equation}
%\resizebox{\textwidth}{!} 
%{$
\mmd(Z,Z') =  \left[\frac{1}{\candSize^2}\sum_{i,j=1}^\candSize k(\bfz_i,\bfz_j)-\nonumber\frac{2}{\candSize\trainSize}\sum_{i,j=1}^{\candSize,\trainSize}k(\bfz_i,\bfz'_j) +\frac{1}{\trainSize^2}\sum_{i,j=1}^\trainSize k(\bfz'_i,\bfz'_j)\right]^\frac{1}{2} 
%$}
\end{equation}
where $k$ is the kernel of the RKHS.
%While this estimate of \(\mmd\) is biased (denoted as \(\mmd_b(Z,Z')\)), it is often used in practice to avoid imaginary results~\cite{gretton2012kernel}.
%We note that the computation cost for both the biased and unbiased estimates are the same~\cite{gretton2012kernel} and minimum variance estimate is almost identical in both cases~\cite{serfling2009approximation}.
%This means that given $Z$ and $Z'$, both the biased and unbiased estimates will be almost identical.
Let $d=\vert \mmd(Z,Z')-\mmd(p,p')\vert$.
Gretton {\em et. al.} show that 
\begin{equation}
P\left(d > 2 \left(\sqrt{\frac{K}{n}} + \sqrt{\frac{K}{m}}\right) + \epsilon \right) \le 2 e^{-\frac{\epsilon^2nm}{2K(n+m)}}
\end{equation}
where $K$ is an upperbound on the kernel values.

We convert the above bound into a one-sided hypothesis testing procedure.
Under the null hypothesis $p=p'$ we have $\mmd(p,p')=0$. 
We consider positive deviations of $\mmd(Z,Z')$ from $\mmd(p,p')$.
Equating the RHS with $\alpha$ (probability of incorrectly stating $p\ne p'$ also known as the type I error) gives a hypothesis test of level-$\alpha$, where solving $\epsilon$ as a function of $\alpha$ gives
$
\alpha = e^{-\frac{\epsilon^2nm}{2K(n+m)}} \Rightarrow \epsilon = \sqrt{\frac{2K(n+m)}{nm}\log\frac{1}{\alpha}}
$.
We retain the null hypothesis if
\begin{equation}
\mmd(Z,Z') - T <0
\end{equation}
where the threshold is
\begin{equation}
%\resizebox{.5\textwidth}{!} 
%{$
T = 2 \left(\sqrt{\frac{K}{n}} + \sqrt{\frac{K}{m}}\right) + \sqrt{\frac{2K(n+m)}{nm}\log\frac{1}{\alpha}}
%$
%}
\end{equation}
This also defines Eve's detection function ($\suspicion(\cand,\trset)$) at level-$\alpha$: 
\begin{equation}
\suspicion(\cand,\trset)\equiv\mmd(\cand,\trset) - T.
\end{equation}
If $\suspicion(\cand,\trset) \ge 0$ then Eve realizes that $\trset$ is not drawn i.i.d. from $\mathbb{\cdist}_{(\bfx, y)}$ and flags it as suspicious.
%Note that, in this setting, $\cand$ is i.i.d. but $\trset$ is usually not.
%Eve's goal is to determine if the camouflaged training set \(\trset\)  comes from a different distribution than the camouflage pool \(\cand\).
%Alice, on the other hand, actively attempts to fool Eve.

%Incorporating \(\mmd\) into Alice's optimization problem yields: 
%\begin{align}
%	\argmin_{D\in 2^\cand} &\frac{1}{|\val|}\sum_{(\tx, \ty)\in \val}\tloss(\learner(D)(\tx), \ty) \nonumber \\
%	\text{s.t.
%} &\mmd_b(\cand,\trset) - 2\left(\sqrt{\frac{K}{\vert\cand\vert}} + \sqrt{\frac{K}{\vert \trset\vert}}\right) \nonumber\\
%	&- \sqrt{\frac{2K(\vert\cand\vert+\vert \trset\vert)}{\vert\cand\vert\vert \trset\vert}\log\frac{1}{\alpha}} < 0~\label{eq:framework}
%\end{align}

%Also note that, since we assume Alice knows Eve's detector function, this implies that she knows the kernel function $k$ and the test level-$\alpha$ used by Eve.
%Keeping these information in mind, Alice attempts to solve the optimization problem in (\ref{eq:framework}).
%We explore this in subsequent sections of the paper.
%We note that it is possible for Eve to use other detector functions.
%The camouflage framework and the solvers will still remain the same even then.

%We now have a fully specified training set camouflage optimization problem~\eqref{aliceopti}.

For all our experiments Eve used the RBF kernel $k(\bfz_i, \bfz_j) = \exp\left(-\frac{\Vert \bfz_i - \bfz_j \Vert^2}{2\sigma^2}\right)$. 
Eve set $\sigma$ to be the median distance between points in the camouflage pool as proposed in ~\cite{gretton2012kernel}. 
Eve also included the scaled class label as a feature dimension: $[\bfx_i, c \mathbbm{1}\{y_i=1\}]$ where
$c=\max_{k,l\text{ such that } y_k = y_l} \Vert \bfx_{k} - \bfx_{l}\Vert$
and $\mathbbm{1}\{\cdot\}$ is the indicator function.
%Thus $c_i$ is $0$ if the label of the instance is not $1$, otherwise the label is scaled by the maximum distance between pairs of points in the same class, $c$. 
%We scaled the label in this manner because it has been found  that the scale of a particular dimension is important while applying a kernel function~\cite{chatfield2011devil}. 
%Note that, this means that if $x_i$ and $x_j$ are in the same class, then $\Vert [\bfx_i, c_iy_i] - [\bfx_j, c_jy_j] \Vert = \Vert \bfx_i - \bfx_j \Vert$. 
%Otherwise, $\Vert [\bfx_i, c_iy_i] - [\bfx_j, c_jy_j] \Vert = \Vert \bfx_i - \bfx_j \Vert + c$. 
%Thus the distance between pairs of points with different labels are increased. 
This augmented feature enables Eve to monitor both features and labels. 
When using the NLP solver Alice only has to consider instances from camouflage pool. 
She calculated $\mmd$ in the following manner:
\begin{align}
%\resizebox{\textwidth}{!} 
%{$
\mmd_b(Z, b_1,\ldots,b_{|Z|})=&\left[\frac{1}{\candSize^2}\sum_{i,j=1}^\candSize k(\bfz_i,\bfz_j) - \frac{2}{n\sum_{i=1}^{\candSize} b_i}\sum_{i,j=1}^{\candSize} b_ik(\bfz_i,\bfz_j)\right.\nonumber\\
& \left.+ \frac{1}{(\sum_{i=1}^{n}b_i)^2} \sum_{i,j=1}^{n} b_ib_jk(\bfz_i,\bfz_j)\right]^\frac{1}{2}
%$}
\end{align}

==> arxiv_Paper (copy)/relwork.tex <==

Concealing the existence of messages is known as steganography. 
%This is different from cryptography where the goal is to conceal the content of messages. 
One illustration of steganography (first presented in 1983 in \cite{simmons1984prisoners}) is where prisoners Alice and Bob wish to devise an escape plan. 
All their communication is observed by the adversary (the warden, Eve) who will thwart their plan as soon as she detects any sign of hidden message. 
%In this setup, the mode of communication is text.
%An information-theoretic model for such a setup is presented in~\cite{cachin1998information}. 
%The theoretical limitation of steganography was explored in \cite{anderson1998limits}. 
%Steganography is done in domain of images as well~\cite{queirolo2011steganography,johnson1998exploring}. 
%More recently it was proposed by the author  of \cite{baluja2017hiding} to hide a full sized image inside another one with the help of deep neural networks. 

Steganography has multiple real-world applications including secret communication~\cite{zhang2009image}, feature tagging elements~\cite{maganbhaistudy}, and copyright protection~\cite{maganbhaistudy}.
Although many different data formats can be used for steganography, images~\cite{queirolo2011steganography,johnson1998exploring} are by far the most popular format due to their popularity on the internet and the fact that they are rich with noise-insensitive information.
Image steganography can be broadly classified into spatial domain, transform domain, spread spectrum and model based \cite{singh2014survey}, and has been thoroughly studied.
%In spatial domain steganography, embedding the secret message is done on the image pixels directly~\cite{johnson1998exploring,wu2003steganographic}.
%For transform domain steganography, embedding the message requires transforming the image from the spatial domain to the frequency domain by using some transformation like discrete cosine transform (DCT)~\cite{bhattacharya2012session}, discrete wavelet transform (DWT)~\cite{gupta2015discrete}, singular value decomposition (SVD)~\cite{hemdan2013efficient} etc.
%The spread spectrum steganography techniques~\cite{marvel1999spread,valizadeh2011correlation} are characterized by their robustness against statistical attacks.
%Model based steganography~\cite{sallee2003model} only alters part of the cover image to carry the secret message without modifying the cover statistical properties.
%This method is relatively new and is also known as adaptive steganography.
On the other side, steganalysis is the study of detecting the existence of hidden messages (using steganography).
Identifying such messages in text by looking at patterns in texts, odd language and unusual white space was explored in~\cite{chandramouli2002mathematical}.
The authors of 
\cite{fridrich2004feature,ker2005steganalysis,queirolo2011steganography} 
%\cite{fridrich2004feature,queirolo2011steganography} 
 explore the detection of hidden messages in images.


A study of steganography from a complexity-theoretic point of view is presented in~\cite{hopper2002provably,reyzin2003more}.
An information-theoretic model for such a setup is presented in~\cite{cachin1998information}. 
This complexity-theoretic security notion is similar to modern cryptography and they try to define a secure stegosystem such that the stegotext is computationally indistinguishable from the covertext.
In such a scenario a new term called steganographic secrecy of stegosystem is introduced which is defined as the inability of a polynomial-time adversary (Eve) to distinguish between observed distributions of unaltered covertext and stegotexts.
%To the best of our knowledge this paper is the first to explore steganographic techniques in the domain of training sets for machine learning models.
To the best of our knowledge, steganographic techniques have not been used in the domain of training sets for machine learning models.


Steganography is often confused with cryptography~\cite{katz1996handbook,van2014encyclopedia}, however the goal of these two systems are completely different. 
The goal of cryptography is to ensure confidentiality of data in communication and storage processes.
Hiding the existence of sensitive data is not the end goal here (unlike steganography). 
According to Kerckhoffs's principle~\cite{kerckhoffs18831,kerckhoffs18832}, this confidentiality must not rely on the obfuscation of the encoding scheme, but only on the secrecy of the decryption key.

%Encryption schemes can be broadly categorized in two ways: symmetric and asymmetric.
%In the symmetric scheme~\cite{mroczkowski2001implementation,daemen2013design,vernam1926cipher,ekdahl2002new} both Alice and Bob share the encryption/decryption key.
%The main advantage of the symmetric schemes is fast computation.
%But its application is limited because Alice and Bob have to determine the key beforehand and also because a separate key is required for interaction between different parties.
%Asymmetric schemes~\cite{rivest1978method,elgamal1985public}, on the other hand, use a separate encryption and decryption key.
%In this scenario Alice uses her \textit{public key} to encrypt the data while Bob uses his \textit{private key} to decrypt it.
%The main advantage of this scheme is that the sender and receiver do not have to agree on anything before passing the the data and hence these are widely used in practice.
%The main disadvantage of this scheme is high computation time.

One particular branch of cryptography we highlight is {homomorphic encryption}~\cite{rivest1978data}.
Consider a situation where you seek to delegate some computation to another computer (e.g., using a cloud computation service to a perform machine learning task).
You would like to utilize their computation power, but you do not trust them with your private data.
Homomorphic encryption allows a method by which you can encrypt your data prior to sending it.
The untrusted computer will then perform its operations on the encrypted data, returning to you the result (e.g., a learned model).
You then decrypt the result, yielding what the remote computer would have computed had you provided your original (unencrypted) data.
A homomorphic cryptosystem which supports arbitrary computation on ciphertexts is known as fully homomorphic encryption (FHE).
The first plausible construction of such a system was proposed in~\cite{smart2010fully}. 
This scheme supports both addition and multiplication operations on ciphertexts, which in turn makes possible to construct circuits for arbitrary computations.
Some second generation solutions were proposed in~\cite{brakerski2014leveled,brakerski2012fully,lopez2012fly,gentry2013homomorphic}.
%\cite{brakerski2014leveled,brakerski2012fully}.

In our setting, encryption (homomorphic or otherwise) is not enough to solve Alice's task.
After Alice has transmitted her data to Bob, Bob learns a model.
Alice's goal is not only for Eve to not know the model (which could easily be achieved by Alice simply sending an encrypted model), but also for Eve not to be suspicious.
Eve believes that Alice is drawing data points i.i.d. from some distribution and thus data encrypted by standard methods will cause alarm.
We do note that the relatively new method of ``honey encryption''~\cite{juels2014honey} may be a useful alternative approach for Alice, which we leave as future work.



\begin{comment}
In asymmetric cryptography schemes~\cite{rivest1978method,elgamal1985public}, Alice and Bob use separate encryption and decryption keys which has led to many applications.
There is another branch of cryptography which deals with performing computation on encrypted data.
One usefulness of such a scheme would be when we delegate some computation to an untrusted computer.
The untrusted computer will perform the computation on encrypted data, hence will not know the real contents of it, and return the computed value.
For coherence, the result sent back by the untrusted computer has to equal to the intended computed value if performed on the original data.
This scheme is known as \textit{homomorphic encryption} and was first proposed by Rivest et al. in 1978~\cite{rivest1978data}.
A homomorphic cryptosystem which supports arbitrary computation on ciphertexts is known as fully homomorphic encryption (FHE).
The first plausible construction of such a system was proposed in~\cite{smart2010fully}. 
This scheme supports both addition and multiplication operations on ciphertexts, which in turn makes possible to construct circuits for arbitrary computations.
Some second generation solutions were proposed in~\cite{brakerski2014leveled,brakerski2012fully,lopez2012fly,gentry2013homomorphic}.
These second generation cryptosystems feature much slower growth of the noise during the homomorphic computations.
We note that the communication problem proposed here between Alice and Bob cannot be solved using cryptography (or homomorphic cryptography).
This is because one of Alice's goals is not to raise Eve's suspicion.
Eve only expects Bob to receive data in a particular format (image, text etc.).
Seeing encrypted data will automatically raise Eve's suspicion and cause Alice to fail in her goal.
\end{comment}


The idea of constructing a dataset keeping a particular machine learning algorithm and a target model in mind is known as machine teaching. 
Machine teaching is the inverse of machine learning and has applications in various fields~\cite{zhang2018training,liu2016teaching}. 
In particular, machine teaching has applications in the domain of adversarial learning which studies the use of machine learning in security-sensitive domains.
Numerous attacks against various machine learners have been explored, highlighting the security ramifications of using machine learning in practice \cite{huang2011adversarial,barreno2006can,barreno2010security,dalvi2004adversarial,laskov2009framework,tan2002undermining}.

In the work presented herein, Alice can be thought of as ``attacking'' the learner Bob, in that she aims to provide a dataset which causes Bob to learn a model with parituclar properties.
We highlight how this differs from the classical adversarial learning framework in two ways.
First, Alice is not perturbing an existing training set, but rather generating one.
Thus, this is more akin to the Machine Teaching framework.
Second is the presence of Eve.
Namely, Alice is trying not only to affect Bob's resulting model, but also to hide her involvement from a third party eavesdropper.
In spirit, this is similar to the adversarial learning work performed on intrusion detection systems~\cite{kloft2007poisoning,kloft2011online}.
In terms of the details of the mathematics, our framework and strategies for solving Alice's optimization problem more closely follow~\cite{mei2015using}.


%On the side of defense, much work has been done in both steganography and adversarial learning.
%Within the realm of steganography, detection of such hidden messages have also been part of ongoing research. 
%Identifying such messages in text by looking at patterns in texts, odd language and unusual white space was explored in~\cite{chandramouli2002mathematical}. 
%Detecting hidden messages in images was explored with the use of statistical analysis in~\cite{queirolo2011steganography}.
%In this paper we explicitly model Eve as an agent aiming to detect Alice's hidden message, and focus on Alice's ability to keep her intentions hidden. 
Within adversarial machine learning, a line of research has posed the problem of learning in the presence of adversaries in game theoretic contexts~\cite{liu2009game,bruckner2012static,dalvi2004adversarial,bruckner2009nash,bruckner2011stackelberg,hardt2016strategic,bruckner2011stackelberg}. 
\cite{dalvi2004adversarial,letchford2013optimal,alfeld2017explicit} specifically address a learner's defense strategy in various contexts.
Randomization has also been explored as a method of defense~\cite{bulo2016randomized,vorobeychik2014optimal}, as well as in the context of machine teaching \cite{balbach2006teaching}.
Our work contributes to this conversation as Eve can be seen as a form of defense for Bob.





==> arxiv_Paper (copy)/solvingopti.tex <==

In this section, we propose three methods of solving the optimization problem defined in (\ref{aliceopti}).
We first show how the optimization problem can be reduced to a nonlinear programming problem for a broad class of learners.
We relax the resulting optimization problem to one which is computationally efficient to solve.
We then present two combinatoric methods as heuristic methods applicable to any learner.

\subsection{Nonlinear Programming (NLP)}\label{sec:NLP}

We assume Bob's machine learning algorithm $\learner$ solves a convex optimization problem.
Specifically, Bob performs  regularized empirical risk minimization.
This covers a wide range of learners such as support vector machines~\cite{hearst1998support}, logistic regression~\cite{hosmer2013applied}, and ridge regression~\cite{hoerl1970ridge}.
Let $\Theta$ be Bob's hypothesis space,  $\closs$ his loss function, and $\lambda$ his regularization parameter, respectively.
%Note that, Bob's loss function may be different from Alice's loss function ($\tloss$). As only Alice has access to the sensitive set, she might want to reduce some particular error on the sensitive set (e.g., 0/1 loss) while Bob's loss might be fixed beforehand (e.g., logistic loss).
%For example, Bob's loss function can be logistic loss function while Alice's loss function is $0/1$ Error.
Let $\trainSize:=\vert \trset \vert$ be given.
We convert Alice's optimization problem~(\ref{aliceopti}) into a nonlinear programming problem as follows.

\textbf{Step 1.} 
Using the definition of Bob, we rewrite~(\ref{aliceopti}) as
\begin{align}
	\min_{\trset\subset \cand, \hat\theta \in \Theta}& ~~&&\frac{1}{\vert \val \vert} \sum_{(\tx, \ty)\in \val}\tloss(\hat{\theta}, \tx, \ty)\nonumber\\
	\text{s.t.}& ~~&&\hat{\theta} = \argmin_{\theta \in \Theta} \sum_{(\bfx, y)\in\trset} \closs(\theta, \bfx, y) + \frac{\lambda}{2} \Vert \theta \Vert^2\nonumber\\
	& &&\suspicion(\cand,D) < 0, \nonumber \\
	& &&\vert \trset \vert = \trainSize.\label{eq:MMDConstraint}
\end{align}
We make note that in both levels of this bilevel optimization problem (the upper and lower levels corresponding with Alice and Bob, respectively) \(\tloss(\cdot)\) is being minimized.
That is, Alice and Bob both seek to minimize the loss of Bob's resulting model.
Due to its combinatorial nature, this is a computationally difficult problem to solve.

\textbf{Step 2.}
Since Bob's learning problem (the lower level optimization problem) is assumed to be convex, satisfying its Karush-Kuhn-Tucker (KKT) conditions is necessary and sufficient for a point to be optimal~\cite{wu2007karush,liu2016teaching}.
Thus we replace the lower level optimization problem in~(\ref{eq:MMDConstraint}) with the KKT conditions to obtain a single-level optimization problem:

\begin{align}
	\min_{\trset\subset \cand, \hat\theta \in \Theta}& ~~&&\frac{1}{\vert \val \vert} \sum_{(\tx, \ty)\in \val}\tloss(\hat{\theta}, \tx, \ty)\nonumber\\
	\text{s.t.}& ~~&& \sum_{(\bfx, y)\in\trset} \triangledown\closs(\hat\theta, \bfx, y) + \lambda\hat\theta = 0,\nonumber\\
	& &&\suspicion(\cand,D) < 0, \nonumber\\
	& && \vert D \vert = \trainSize.
\end{align}
While now a single level optimization problem, selecting a subset $\trset\subset \cand$ is still a combinatorial problem and computationally expensive to solve.
In what comes next we relax this problem to one of continuous optimization.

\textbf{Step 3.}
We introduce binary indicator variable $b_i$ for each instance $(\bfx_i, y_i) \in \cand$.
A value of \(1\) indicates that the instance is a member of the training set \(D\).
Also dropping the hat on $\hat\theta$ for simplicity.
This yields:
\begin{align}
	\min_{\theta \in \Theta;b_1,\ldots,b_{|\cand|};b_i \in \{0, 1\}} ~~\frac{1}{\vert \val \vert} \sum_{(\tx, \ty)\in \val}{\tloss(\theta, \tx, \ty)} \nonumber\\
	\text{s.t.} ~~\sum_{i=1}^{\candSize} b_i\triangledown\closs(\theta, \bfx_i, y_i) + \lambda\theta = 0,\nonumber\\
	\suspicion(\cand,\{b_i(\bfx_i, y_i)|(\bfx_i,y_i)\in\cand,b_i\ne 0\}) < 0\nonumber\\
	\sum_{i=1}^{\candSize}b_i = \trainSize.
\end{align}
This is known as a Mixed Integer Non-Linear Optimization Problem (MINLP)~\cite{bussieck2003mixed}.
MINLP problems are generally hard to solve in practice. 
However, phrasing the problem in this way yields a natural relaxation.
Namely we relax $b_i$ to be continuous in $[0,1]$, resulting in the following non-linear optimization problem:
\begin{align}
	\min_{\theta \in \Theta;b_1,\ldots,b_{\candSize} \in [0, 1]} ~~\frac{1}{\vert \val \vert} \sum_{(\tx, \ty)\in \val}{\tloss(\theta, \tx, \ty)} \nonumber\\
	\text{s.t.} ~~\sum_{i=1}^{\candSize} b_i\triangledown\closs(\theta, \bfx_i, y_i) + \lambda\theta = 0,\nonumber\\
	\suspicion(\cand,b_1,\ldots,b_{|\cand|}) < 0,\nonumber\\
	\sum_{i=1}^{\candSize}b_i = \trainSize.
\end{align}
Note that in this equation we scale the gradient of the loss function for each $(\bfx_i, y_i)$ by the corresponding $b_i$.
This $b_i$ indicates the importance of an instance in the training set.
In essence, the learner is training on a ``soft'' version of the dataset, where each training example is weighted.
Similarly, when calculating the detection function we weigh each instance in the training set by its corresponding $b_i$.
The exact nature of this weighing depends on the detection function itself.
We further note that the nonlinear optimization problem is non-convex.
As such, Alice must seed her solver with some initial $\{b_i\}$.
This is discussed further in Section~\ref{sec:exp}.

After solving this (continuous) optimization problem, Alice must round the $\{b_i\}$'s into binary indicators so that she can select a training set to send to Bob.
Alice uses a rounding procedure that proposes $m+1$ candidate training sets $D^{(1)}, \ldots, D^{(m+1)}$ from the continuous solution $\{b\}$.
The candidate training sets include 
(1) the training set $D^{(1)}$ consisting of the $m$ items with the largest $b$ values, 
(2) the seed training set before running optimization, 
(3) $m-1$ other training sets that ``interpolate'' between 1 and 2.
Alice then checks $D^{(1)}, \ldots, D^{(m+1)}$ for feasibility (satisfying $\suspicion$) and picks the best one. 
Note the seed training set is feasible, hence Alice is guaranteed to have a solution.
The interpolation scheme ensures that Alice will find a solution no worse than the seed set.

Concretely, let $S$ be the $m$-item seed training set and $\cand \backslash S$ be the remaining items.
Alice sorts items in $S$ by their $b$ values.
Separately, Alice sorts items in $\cand \backslash S$ by their $b$ values.
Then, Alice starts from $S$ and sequentially swaps the least-valued item in $S$ with the largest-valued item in $\cand \backslash S$.
She performs $m$ swaps.  This produces the $m+1$ candidate training sets, including the original $S$.
It can be shown that the $m$ items with the largest $b$ values will be one of the training sets.


% The Alice who used the NLP solver seeded the solver with the camouflaged training set found during the candidate task identification phase.
% After running the solver she also evaluated a further $m$ training sets as part of the rounding procedure.
% Let $I$ and $N$ identify the index vector of all instances in the initial dataset and all other instances in the camouflage pool respectively. 
% Also let, $I'$ and $N'$ represent the sorted sequence of $I$ and $N$ such that $b_{I'_i} \ge b_{I'_i+1}$ and $b_{I'_i} \ge b_{I'_i+1}$. Now we define,
% $T_c=[I'_1,I'_2,\ldots,I'_{m-c},N'_1,N'_2,\ldots,N'_c]$.  
% Here $c\in\mathbb{Z}: c\in[0,m]$. 
% Thus $T_0=I'$ and $T_m=[N'_1,N'_2,\ldots,N'_m]$.
% Alice evaluates the training sets $\cand_{T_c}$ for all values of $c$. 
% Note that she does not need to re-evaluate $T_0$. Thus the camouflaged training set found by using the NLP solver is:
% \begin{align}
% \argmin_{c\in\mathbb{Z}: c\in[0,m]}& ~~&&\frac{1}{\vert \val \vert} \sum_{(\tx, \ty)\in \val}\tloss(\hat{\theta}, \tx, \ty)\nonumber\\
% \text{s.t.}& ~~&&\hat{\theta} = \argmin_{\theta \in \Theta} \sum_{(\bfx, y)\in\cand_{T_c}} \closs(\theta, \bfx, y) + \frac{\lambda}{2} \Vert \theta \Vert^2\nonumber\\
% & &&\suspicion(\cand,\cand_{T_c}) < 0
% \end{align}


\subsection{Uniform Sampling}

For any learner Bob, even one which does not solve a convex empirical risk minimizing problem discussed above, Alice has a simple option for finding a training set.
Let Alice's budget \(\tb\) denote the number of times Alice is able to train the classifier $\learner$.
She first creates \(\tb\) training sets $D^{(1)}, \ldots, D^{(\tb)}$, each by sampling $m$ points uniformly without replacement from her camouflage pool $\cand$, such that each $D^{(j)}$ successfully bypasses Eve i.e., $\suspicion(\cand, D^{(j)})<0$.
%She then tests to see if each $D^{(j)}, j=1\ldots \tb$ satisfies $\suspicion(\cand, D)<0$ (the sets that successfully bypass Eve).
Among these $B$ training sets, she then picks the $D^{(j)}$ with the lowest objective value in~\eqref{aliceopti}.
This procedure captures what Bob would learn if given each feasible training set.

\subsection{Beam Search}~\label{sec:search}

%For Bob with a general learner that cannot be formulated as convex empirical risk minimization,
We now describe a heuristic beam search algorithm~\cite{rich1991artificial} to approximately solve Alice's optimization problem~\eqref{aliceopti}.
This process is similar to uniform sampling, described above, but instead of independently generating a new training set every time, Alice performs a local search to augment a proposed training set incrementally.


The state space consists of all training sets $\optSeq\subset \cand$ such that $\vert \optSeq \vert = \trainSize$ and $\suspicion(\cand, \optSeq) < 0$. 
Two training sets that differ by one instance are considered neighbors. 
For computational efficiency, we do not consider the entire set of neighbors at each step.
Instead, we evaluate a randomly selected subset of neighbors for each training set in the beam.
The beam \(\mathcal{D}\) is initialized by selecting \(w\) training sets at random.
The width ($w$) of the beam is fixed beforehand.
From the union of evaluated neighbors and training sets in the current beam, we select the top $w$ training sets (based on the value of the objective function in (\ref{aliceopti})) to reinitialize the beam and discard the rest.
Note that training sets which would be flagged by Eve are not present in the statespace (because Alice has full knowledge of Eve, she need not consider any set that Eve would reject).
We continue the search process until a pre-specified search budget $B$ (number of times the classifier $\learner$ is trained) is met.
Algorithm~\ref{alg:BeamSearch} shows the search procedure with random restarts.

%To formally define the search space, we let the states and neighbor hood function be defined as follows:
%\begin{itemize}
%	\item States: Any training set $(\optSeq)$ such that $\vert \optSeq \vert = \trainSize, \optSeq \subset \cand$
%	\item Initial States: Randomly selected training sets of size $\trainSize$
%	\item Neighbors of a Training Set \(\trset\): All training sets of size $\trainSize$ that differ by one instance with $\trset$. For practical purposes we restrict ourselves to a randomly selected subset of all neighbors.
%\end{itemize}

\begin{algorithm}[htb]
	\caption{Beam Search for Solving the Camouflage Problem}\label{alg:BeamSearch}
	\begin{algorithmic}[1]
		\STATE{Input: Camouflage Pool: $\cand$, Risk: $\mathcal{L}_\learner$, Beam Width: $w$, Budget: $B$, Neighborhood Function: $\mathcal{N}$, Size: $\trainSize$, Detection Function: $\suspicion$, Restarts: $R$ }
		\FOR{$r = 1 \to R$ }
		\STATE{$\mathcal{D}\leftarrow$ $w$ randomly selected subsets of size $\trainSize$ from $\cand$ such that $\suspicion(\cand,D)<0$}
		%\STATE{$\mathbf{D} \leftarrow \argmin_{D\in \mathcal{D}} \mathcal{L}_\learner(D)$}
		\WHILE{budget $B/R$ not exhausted}
			\STATE{$\mathcal{D} \leftarrow \mathcal{D} \cup \mathcal{N}(\mathcal{D},\cand, \suspicion)$, the neighbors}
			\STATE{$\mathcal{D}\leftarrow w$ training sets from $\mathcal{D}$ with smallest $\mathcal{L}_\learner(D)$ values}
			%\STATE{$\mathbf{D} \leftarrow \argmin_{D\in \mathcal{D}} \mathcal{L}_\learner(D)$}
		\ENDWHILE
		\ENDFOR
		\RETURN{the best $D$ found within total budget}
	\end{algorithmic}
\end{algorithm}





==> conc.tex <==

We introduced the training set camouflage setting where a carefully constructed training set can be sent over an open channel with the intention of training a machine learner on a secret classification task.
Using this framework, an agent can hide the intention of the secret task from a third party observer.
We formulated training set camouflage as a bilevel optimization problem and provided methods to approximately solve it based on non-linear programming and combinatorial search.

We conducted empirical experiments on logistic regression and artificial neural network learners with real-world data to see if such a subterfuge is actually possible.
Our results suggest that it is indeed possible to approximately recover the classifier on the original task.
%Among the proposed solvers beam search performed the best overall and is applicable for a wide range of learners.
%Thus beam search should be the preferred solver for Alice.
Among the proposed solvers NLP performed the best overall.

%In some cases, we even get identical results that was found after training on the secret set as well. 
%The present paper should serve as a warning on the existence of such camouflage attacks.

In the future, we plan to devise defensive mechanisms to detect such subterfuge.
We also plan to explore training set camouflage in a cross modality domain (e.g., when the secret task is text classification while the camouflage task is image classification) and in settings where Alice does not have complete information about Eve or Bob.
We also intend to further investigate Alice's capability to remain undetected while altering Bob's learned model in a training-time attack setting, where Alice perturbs an already existing training set, rather than creating one.




==> exp.tex <==

We investigated the effectiveness of training set camouflage through empirical experiments on real world datasets. 
Our results show that camouflage works on a variety of image and text classification tasks: 
Bob can perform well on the secret task after training on the camouflaged training set,
and the camouflaged training set passes Eve's test undetected.

\textbf{Bob}.  We considered two different learning algorithms for Bob: logistic regression and artificial neural network (ANN)~\cite{karabatak2009expert}.
Both of these learners are popular and regularly used in practice. 
For the logistic regression learner, the weight of the regularization parameter was set to $1$. 
We present the specification and results for the ANN in Appendix B.

\textbf{Eve}.
For our experimental purposes we used Maximum Mean Discrepancy ({\mmd})~\cite{gretton2012kernel} as Eve's detection function.
{\mmd} is a widely used two-sample test~\cite{dziugaite2015training} but cannot be directly used in the camouflage framework.
\todo{you have to briefly say why.   also this directly contradicts with the first sentence "we used MMD"}
We introduce {\mmd} and Eve used it in Appendix A.
The level-$\alpha$ for this detection function was set to $0.05$ (i.e., 95\% confidence). 


\textbf{Alice}.
%For the ANN Bob, Alice only used beam search and uniform sampling (nonconvexity prevents application of KKT); while for logistic regression she used all three  solvers. 
Alice constructed camouflaged training sets of size $m=20$, $100$ and $500$.
For all secret tasks Alice was allotted separate budgets to identify a suitable camouflage task and then the camouflaged training set.
Alice used uniform sampling with a search budget of $80,000$ to identify a suitable camouflage pool.
This meant that Alice stopped the search after training the logistic regression learner $80,000$ times.
For simplicity we assume that during this phase $m$ was set to $20$ for all cases.
Alice had a further budget of $80,000$ to find a camouflaged training set for both beam search and uniform sampling.
For beam search, she performed five random restarts each with a budget of $16,000$ and then used the best found training set.
Here the size of the beam was $10$ and for each training set in the beam, $50$ randomly selected neighbors were evaluated during each iteration.
%For beam search, the search budget was set to $200,000$, then repeated five times with random restarts.
%This meant that Alice stopped the search for a camouflaged training set after training the learner $200,000$ times.
The NLP solver does not have a notion of budget and Alice must seed the solver with some initial dataset.
Thus it cannot be directly compared with the other two solvers.
Alice performed a separate experiment with only $m=20$.
In this case the initial dataset was set to be the output found by the beam search solver.
The loss $\ell$ was logistic loss and squared loss for logistic regression and ANN, respectively. 


\textbf{Evaluation metrics}.
As is standard to estimate general performance, we used a separate test set, generated from the same distribution as the secret set $D_S$ and not known to any agent, to evaluate Bob's generalization error when trained on Alice's camouflaged training set $D$.
We compare this to two quantities:
(``random'') when Bob is trained on a uniform sample of size $m$ from the cover data distribution, which we expect to perform poorly; and 
(``oracle'') when Bob is trained directly on Alice's secret set $D_S$, ignoring Eve's presence.
The oracle gives us an estimate on how much performance Bob is losing due to camouflage.


\subsection{Datasets}

%We performed eight camouflage experiments: WM71, WMOA, GP52, GPOA, CABH, CAIM, DRBH and DRIM as described below.
%The first two letters in the acronyms encode the secret task, and the last two the cover task.
%In both WM71 and WMOA the secret task was woman vs. man (CIFAR-100), the cover task was handwritten digits 7 vs. 1 (MNIST) and orange vs. apple (CIFAR-100), respectively. 
%In GP51 and GPOA the secret task was handgun vs. phone image classification (OpenImages~\cite{openimages}),
%the cover was 5 vs 1 and orange vs. apple, respective.
%In CABH and CAIM the secret task was text classification on christian vs atheism (20-newsgroups), the cover tasks were baseball vs hockey and pc vs mac, respectively.
%In DRBH and DRIM the secret task was text classification on Democratic vs. Republican , the cover tasks were baseball vs hockey and pc vs mac, again.
%For all datasets, the positive/negative examples of the sensitive set were mapped to the positive/negative examples of the camouflage pool.
%We do so because we assume that Alice is not allowed to modify instances in the camouflage pool.
%Since Eve also has access to the same camouflage pool, such modifications will be easy to detect for her.

%We performed experiments for four secret tasks: women vs. man (CIFAR-100) images (WM), handgun vs. phone (OpenImages~\cite{openimages}) images (GP), christian vs. atheism (20-newsgroups) articles (CA) and Democratic vs. Republican (All The News dataset~\cite{allthenews2017}) articles (DR).
We performed experiments for four secret tasks: WM (CIFAR-100~\cite{krizhevsky2009learning}), GP (OpenImages~\cite{openimages}), CA (20-newsgroups~\cite{joachims1996probabilistic}) and DR (All The News dataset~\cite{allthenews2017}).
The two letters in the acronym represent the two classes in the corresponding task.
The first two tasks were image classification while the remaining two were text classification.
For the image tasks we selected eight candidate cover tasks. 
Six of them were from the MNIST handwritten digits: 17, 71, 25, 52, 69 and 96.
The other two were from the CIFAR-100 dataset: OA and OA.
Similarly for the text tasks we also selected eight candidate cover tasks.
All of them were from the 20-newsgroups dataset: BS, HB, IM, MI, AM, MA, MX and XM.
As before the acronyms here represent the class names.


For images we used ResNet~\cite{he2016deep} to generate feature vectors of dimension $2048$. 
For text we used Word2Vec~\cite{mikolov2013efficient} to generate feature vectors of dimension $300$ by averaging over the word vectors in an article.
A summary of the sensitve sets and camouflage pools (along with the corresponding classes) can be found in Table~\ref{tab:dataSum}.

%\begin{table*}[!htb]
%	\centering
%	\caption{Dataset Summary}~\label{tab:dataSum}
%	\resizebox{\textwidth}{!}{%
%	\begin{tabular}{|l|l|r|r|r|r|r|r|r|}
%		\hline
%		\multicolumn{1}{|c|}{\textbf{Name}} & \multicolumn{1}{|c|}{\textbf{Type}} & \multicolumn{1}{|c|}{\textbf{\# Features}} & \multicolumn{1}{|c|}{\textbf{\# Camouflage }} & \multicolumn{1}{|c|}{\textbf{\# Camouflage }} & \multicolumn{1}{|c|}{\textbf{\# Secret }} & \multicolumn{1}{|c|}{\textbf{\# Secret }} & \multicolumn{1}{|c|}{\textbf{\# Test }} & \multicolumn{1}{|c|}{\textbf{\# Test }} \\
%		 &  &  & \multicolumn{1}{|c|}{\textbf{Pool Positive}} & \multicolumn{1}{|c|}{\textbf{Pool Negative}} & \multicolumn{1}{|c|}{\textbf{Positive}} & \multicolumn{1}{|c|}{\textbf{Negative}} & \multicolumn{1}{|c|}{\textbf{Positive}} & \multicolumn{1}{|c|}{\textbf{Negative}} \\
%		\hline
%		WM71 & Image & $2048$ & $600$ & $600$ & $500$ & $500$ & $100$ & $100$ \\\hline
%		WMOA & Image & $2048$ & $600$ & $600$ & $500$ & $500$ & $100$ & $100$ \\\hline
%		GP52 & Image & $2048$ & $600$ & $600$ & $400$ & $400$ & $100$ & $100$ \\\hline
%		GPOA & Image & $2048$ & $600$ & $600$ & $400$ & $400$ & $100$ & $100$ \\\hline
%		CABH & Text & $300$ & $994$ & $999$ & $599$ & $480$ & $398$ & $319$ \\\hline
%		CAIM & Text & $300$ & $982$ & $963$ & $599$ & $480$ & $398$ & $319$  \\\hline
%		DRBH & Text & $300$  & $994$  & $999$ & $800$ & $800$ & $200$ & $200$ \\\hline
%		DRIM & Text & $300$  & $982$ & $963$ & $800$ & $800$ & $200$ & $200$ \\\hline
%	\end{tabular}
%	}
%\end{table*}

%\begin{table*}[!htb]
%	\centering
%	\caption{Dataset Summary}~\label{tab:dataSum}
%	\resizebox{\textwidth}{!}{%
%		\begin{tabular}{|l|l|r|r|r|r|r|r|r|}
%			\hline
%			\multicolumn{1}{|c|}{\textbf{Name}} & \multicolumn{1}{|c|}{\textbf{Type}} & \multicolumn{1}{|c|}{\textbf{\# Features}} & \multicolumn{1}{|c|}{\textbf{\# Camouflage }} & \multicolumn{1}{|c|}{\textbf{\# Camouflage }} & \multicolumn{1}{|c|}{\textbf{\# Secret }} & \multicolumn{1}{|c|}{\textbf{\# Secret }} & \multicolumn{1}{|c|}{\textbf{\# Test }} & \multicolumn{1}{|c|}{\textbf{\# Test }} \\
%			&  &  & \multicolumn{1}{|c|}{\textbf{Pool Positive}} & \multicolumn{1}{|c|}{\textbf{Pool Negative}} & \multicolumn{1}{|c|}{\textbf{Positive}} & \multicolumn{1}{|c|}{\textbf{Negative}} & \multicolumn{1}{|c|}{\textbf{Positive}} & \multicolumn{1}{|c|}{\textbf{Negative}} \\
%			\hline
%			%WM71 & Image & $2048$ & $600$ & $600$ & $500$ & $500$ & $100$ & $100$ \\\hline
%			WMOA & Image & $2048$ & $600$ & $600$ & $500$ & $500$ & $100$ & $100$ \\\hline
%			GP96 & Image & $2048$ & $600$ & $600$ & $400$ & $400$ & $100$ & $100$ \\\hline
%			%GPOA & Image & $2048$ & $600$ & $600$ & $400$ & $400$ & $100$ & $100$ \\\hline
%			CABH & Text & $300$ & $994$ & $999$ & $599$ & $480$ & $398$ & $319$ \\\hline
%			%CAIM & Text & $300$ & $982$ & $963$ & $599$ & $480$ & $398$ & $319$  \\\hline
%			DRBH & Text & $300$  & $994$  & $999$ & $800$ & $800$ & $200$ & $200$ \\\hline
%			%DRIM & Text & $300$  & $982$ & $963$ & $800$ & $800$ & $200$ & $200$ \\\hline
%		\end{tabular}
%	}
%\end{table*}

\begin{table}
	\centering
	\caption{Summary of secret sets and camouflage pools.}~\label{tab:dataSum}
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		\textbf{Dataset} & \textbf{Type} & \textbf{\# Features} & \textbf{class 1} & \textbf{class 2} & \textbf{\# class 1} & \textbf{\# class 2} \\\hline
		WM & Image & 2048 & \textbf{w}oman & \textbf{m}an & 500 & 500 \\\hline
		GP & Image & 2048 & hand\textbf{g}un & \textbf{p}hone & 400 & 400 \\\hline
		CA & Text & 300 & \textbf{c}hristian & \textbf{a}theist & 599 & 480 \\\hline
		DR & Text & 300 & \textbf{d}emocratic & \textbf{r}epublican & 800 & 800 \\\hline
		17 & Image & 2048 & digit \textbf{1} & digit \textbf{7} & 600 & 600 \\\hline
		25 & Image & 2048 & digit \textbf{2} & digit \textbf{5} & 600 & 600 \\\hline
		69 & Image & 2048 & digit \textbf{6} & digit \textbf{8} & 600 & 600 \\\hline
		OA & Image & 2048 & \textbf{o}range & \textbf{a}pple & 600 & 600 \\\hline
		BH & Text & 300 & \textbf{b}aseball & \textbf{h}ockey & 994 & 999 \\\hline
		IM & Text & 300 & \textbf{i}bm & \textbf{m}ac & 982 & 963 \\\hline
		AM & Text & 300 & \textbf{a}utos & \textbf{m}otorcycles & 990 & 996 \\\hline
		MX & Text & 300 & \textbf{m}s-windows & windows \textbf{x} &985 & 988 \\\hline
	\end{tabular}
\end{table}


%The formation of the sensitive sets, camouflage pools and test sets are described as follows.
%In both the WM71 and WMOA datasets, the sensitive sets were comprised of images from the popular CIFAR-100 datasets. 
%The classification task was to differentiate between woman and man images. 
%%The training and test images of woman and man found in the CIFAR-100 dataset formed the sensitive set and test set respectively. 
%For the candidate pool of WM71, we used the popular MNIST dataset. 
%The only digits used were $7$ and $1$. 
%We sampled $600$ images at random to generate the camouflage pool. 
%For WMOA dataset, the camouflage pool was created by combining the orange and apple images from CIFAR-100. 
%OpenImages~\cite{openimages} is a well known dataset for image classification tasks. 
%For GP52 and GPOA, we selected $400$ images each at random from the classes Handgun and Mobile Phone to form the sensitive set. 
%A further $100$ images (no overlap with sensitive set) for each class were selected in a similar manner to form the test set. 
%The camouflage pool for GP52 was formed in the same manner as in WM71 except that the images used were $5$ and $2$. 
%The camouflage pool for GPOA was the same as for WMOA.
%
%20 Newsgroups is a popular text dataset. 
%The classification task for CABH and CAIM were to differentiate between articles with labels soc.religion.christian and alt.atheism. 
%The camouflage pool for CABH was created from articles with labels rec.sport.baseball and rec.sport.hockey. 
%Similarly, the camouflage pool for CAIM was created from articles with labels comp.sys.ibm.pc.hardware and comp.sys.mac.hardware.
%All the news is a text dataset~\cite{allthenews2017} that contains news articles from different sources like Breitbart, Washington Post, Fox News etc. 
%Some of these news articles are traditionally leaning towards the Grand Old Party (Republican) while others towards the Democratic Party. 
%In particular, we identified articles published in Breitbart and Fox News to be leaning towards Republicans while articles published in CNN and Washington Post were identified to be Democratic leaning. 
%We sampled $800$ such articles from each group to form the sensitive set for both DRBH and DRIM. 
%Further $200$ articles (no overlap with sensitive set) from each group were sampled to form the test set. 
%The camouflage pools were the same as in CABH and CAIM respectively. 	 

Alice first selected a suitable camouflage pool for each of the secret tasks.
For each candidate task she used a search budget of $10,000$ (allotted a total of $80,000$ budget).
The results of this phase are shown in Table~\ref{tab:imageCandSelect} and \ref{tab:textCandSelect}.
It can be seen that the camouflage pools selected for WM, GP, CA and BH are OA, 96, BH and BH respectively.
The top three camouflaged training sets for GP identified during this phase is shown in Figure~\ref{fig:candidateCover}.

\begin{table}[!htb]
	\centering
	\caption{Logistic loss ($\frac{1}{|D_S|}\sum_{(\tx,\ty)\in D_S}\log(1+\exp(-\ty w^\top\tx))$) after performing uniform sampling search with $m=20$ and search budget $10,000$ for image secret tasks. The best results for each secret task is shown in bold.}~\label{tab:imageCandSelect}
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
		\hline
		\backslashbox{Secret}{Camouflage}
		&\makebox[2em]{17}&\makebox[2em]{71}
		&\makebox[2em]{25}&\makebox[2em]{52} &\makebox[2em]{69}&\makebox[2em]{96}
		&\makebox[2em]{OA}&\makebox[2em]{AO}\\\hline 
		%& 17 & 71 & 25 & 52 & 69 & 96 & OA & AO \\\hline
		WM & $0.790$ & $0.611$ & $0.672$ & $0.688$ & $0.798$ & $0.679$ & $\mathbf{0.584}$ & $0.731$ \\\hline
		GP & $0.480$ & $0.510$ & $0.433$ & $0.390$ & $0.632$ & $\mathbf{0.337}$ & $0.510$ & $0.531$ \\\hline
	\end{tabular}
\end{table}

\begin{table}[!htb]
	\centering
	\caption{Logistic loss after performing uniform sampling search with $m=20$ and search budget $10,000$ for text secret tasks. The best results for each secret task is shown in bold.}~\label{tab:textCandSelect}
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
		\hline
		\backslashbox{Secret}{Camouflage}
		&\makebox[2em]{BH}&\makebox[2em]{HB}
		&\makebox[2em]{IM}&\makebox[2em]{MI} &\makebox[2em]{AM}&\makebox[2em]{MA}
		&\makebox[2em]{MX}&\makebox[2em]{XM}\\\hline 
		%& 17 & 71 & 25 & 52 & 69 & 96 & OA & AO \\\hline
		CA & $\mathbf{0.672}$ & $0.673$ & $0.676$ & $0.675$ & $0.676$ & $0.674$ & $0.675$ & $0.675$ \\\hline
		DR & $\mathbf{0.681}$ & $0.684$ & $0.682$ & $0.683$ & $0.682$ & $0.682$ & $0.682$ & $0.683$ \\\hline
	\end{tabular}
\end{table}

\begin{figure}[htb]
	\centering
	\begin{subfigure}[t]{0.8\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/openimages_sample.pdf}
		\caption{Samples from the secret task Gun vs. Phone (GP)}~\label{fig:GP}
	\end{subfigure}
	
	\begin{subfigure}[t]{0.8\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/GP96.pdf}
		\caption{Camouflaged training set using 9 vs. 6}~\label{fig:GP96}
	\end{subfigure}
	
	\begin{subfigure}[t]{0.8\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/GP52.pdf}
		\caption{Camouflaged training set using 5 vs 2}~\label{fig:GP52}
	\end{subfigure}
	\begin{subfigure}[t]{0.8\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/GP25.pdf}
		\caption{Camouflaged training set using 2 vs. 5}~\label{fig:GP25}
	\end{subfigure}
	\caption{Samples of GP secret set, and the top three camuflaged training set found during the candidate selection phase.}~\label{fig:candidateCover}
\end{figure}


%\begin{table}
%	\centering
%	\caption{Number of models trained per hour for logistic regression learner using Random Argmin search. Total number of models trained (on a $8$ core machine) for individual experiments is $10000$.}
%	\begin{tabular}{|c|c|c|}
%		\hline
%		Dataset & $100$ & $500$ \\\hline
%		WM17 & $243,063$ & $73,099$ \\\hline
%		CABH & $250,963$ & $158,469$  \\\hline
%	\end{tabular}
%\end{table}

%\begin{table}
%	\centering
%	\caption{Number of models trained per hour for ANN learner using Random Argmin search. Total number of models trained (on a $8$ core machine) for individual experiments is $10000$.}
%	\begin{tabular}{|c|c|c|c|}
%		\hline
%		Dataset & $20$ & $100$ & $500$ \\\hline
%		WM17 & $15,272$ & $12,939$ & $8,435$  \\\hline
%		CABH & $15,764$ & $15,223$ & $12,474$ \\\hline
%	\end{tabular}
%\end{table}

\subsection{Results}
We present our results for beam search and uniform sampling in Figure~\ref{fig:lr_results}.
%In this figure, we also show the random error and the oracle error as well for comparison.
%For brevity, we only show $\trainSize=20$ and $\trainSize=500$ results respectively for the image and text datasets.
%But we note that the results presented herein are representative of all experiments performed.
%For the image and text datasets we only show the results when $\trainSize=20$ and $\trainSize=500$ respectively for brevity.
%For the ANN we only used the beam search solver as the NLP solver is not applicable.
%This is because for this learner the NLP solver is not applicable.
%For brevity, we only show $\trainSize=20$ and $\trainSize=500$ results respectively for the image and text experiments.
%But we note that the results presented herein are representative of all experiments performed.
%Each of these figures show the results for one particular $m$ value (20, 100 or 500).
We observe that Alice, using either solver can find much better camouflage training sets than random and in many cases approach oracle.
Keep in mind that Alice's solutions do not trigger Eve's suspicion function.
This shows that such subterfuges are plausible in practice and can actually yield good results from Alice's point of view.


%We show the test error rate after Bob is trained on the sensitive set (baseline error) and also when Bob is trained on the camouflaged training set. Moreover, we also show the length of the training set along with value produced by Eve's detector function (always negative) for our solvers. Looking at the results it can be seen that the test error rate found by both NLP and beam search are relatively close to the baseline error. This is particularly true for the logistic regression learner (note that, for neural network learner we had a reduced search budget). 

%\begin{figure}[!htb]
%	\centering
%	\begin{subfigure}[t]{0.45\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{figures/lr_error_bars.pdf}
%		\caption{Logistic Regression Learner}
%	\end{subfigure}
%	\begin{subfigure}[t]{0.45\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{figures/nn_error_bars.pdf}
%		\caption{Artificial Neural Network Learner}		
%	\end{subfigure}
%	\caption{Test error rates found by solving the camouflage framework. We also show random (with error bars) and oracle error for comparison. For image and text datasets we show results for $\trainSize=20$ and $\trainSize=500$ respectively for brevity.}~\label{fig:results}
%\end{figure}

\begin{figure}[!htb]
	\centering
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/lr_error_bars_20.pdf}
		\caption{$m=20$}
	\end{subfigure}
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/lr_error_bars_100.pdf}
		\caption{$m=100$}
	\end{subfigure}
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/lr_error_bars_500.pdf}
		\caption{$m=500$}
	\end{subfigure}
	\caption{Test error rates found by solving the camouflage framework for the logistic regression learner using beam search and uniform sampling. We also show random (with error bars) and oracle error for comparison.}~\label{fig:lr_results}
\end{figure}




%\begin{table*}[!htb]
%	\centering
%	\caption{Test error rate found by solving the camouflage problem. For image and text datasets we show results of length $20$ and $500$ respectively }~\label{tab:results}
%	%\resizebox{\textwidth}{!}{%
%		\begin{tabular}{|l|r|r|r|r||r|r|r|}
%			\hline
%			\textbf{Name} & \multicolumn{4}{|c||}{\textbf{Bob=Logistic Regression}} & \multicolumn{3}{|c|}{\textbf{Bob=Neural Network}}\\\cline{2-8}	
%			& \multicolumn{1}{|c|}{\textbf{Baseline}} & \multicolumn{1}{|c|}{\textbf{NLP}}  & \multicolumn{1}{|c|}{\textbf{Beam Search}} & \textbf{Oracle} & \multicolumn{1}{|c|}{\textbf{Baseline}} & \multicolumn{1}{|c|}{\textbf{Beam Search}} & \textbf{Oracle} \\
%			& \multicolumn{1}{|c|}{\textbf{Error}} & \multicolumn{1}{|c|}{\textbf{Error}} & \multicolumn{1}{|c|}{\textbf{Error}}& \multicolumn{1}{|c||}{\textbf{Error}}& \multicolumn{1}{|c|}{\textbf{Error}}& \multicolumn{1}{|c|}{\textbf{Error}}& \multicolumn{1}{|c|}{\textbf{Error}}\\\hline
%			WM71 & $0.402 (0.009)$ & $0.335$ & $0.255$ & $0.185$ & $0.452 (0.018)$ & $0.280$ & $0.160$ \\\hline
%			WMOA & $0.426 (0.012)$ & $0.310$ & $0.265$ & $0.185$ & $0.460 (0.013)$ & $0.265$ & $0.160$ \\\hline
%			GP52 & $0.482 (0.031)$ & $0.065$ & $0.025$ & $0.030$ & $0.499 (0.015)$ & $0.115$ & $0.055$ \\\hline
%			GPOA & $0.488 (0.016)$ & $0.340$ & $0.045$ & $0.030$ & $0.528 (0.029)$ & $0.120$ & $0.055$ \\\hhline{|=|=|=|=|=||=|=|=|}
%			CABH & $0.454 (0.002)$ & $0.243$ & $0.255$ & $0.162$ & $0.450 (0.002)$ & $0.278$ & $0.144$ \\\hline
%			CAIM & $0.449 (0.002)$ & $0.240$ & $0.259$ & $0.162$ & $0.460 (0.010)$ & $0.339$ & $0.144$ \\\hline
%			DRBH & $0.497 (0.005)$ & $0.300$ & $0.273$ & $0.243$ & $0.473 (0.006)$ & $0.368$ & $0.248$ \\\hline
%			DRIM & $0.495 (0.006)$ & $0.298$ & $0.303$ & $0.243$ & $0.500 (0.006)$ & $0.353$ & $0.248$ \\\hline
%		\end{tabular}%}
%\end{table*}


%\begin{table*}[!htb]
%	\centering
%	\caption{Best test error rate found. We also show the corresponding length of the camouflaged training set and value of the detector function along with the baseline test error rate}
%	\resizebox{\textwidth}{!}{%
%	\begin{tabular}{|l|r|r|r|r|r|r|r||r|r|r|r|}
%		\hline
%		\textbf{Name} & \multicolumn{7}{|c||}{\textbf{Logistic Regression}} & \multicolumn{4}{|c|}{\textbf{Neural Network}}\\\cline{2-12}	
%		& \textbf{Baseline} & \multicolumn{3}{|c|}{\textbf{NLP}}  & \multicolumn{3}{|c||}{\textbf{Beam Search}} & \textbf{Baseline} & \multicolumn{3}{|c|}{\textbf{Beam Search}} \\\cline{3-8}\cline{10-12}
%		& \multicolumn{1}{|c|}{\textbf{Error}} & \multicolumn{1}{|c|}{\textbf{Error}} & \multicolumn{1}{|c|}{\textbf{Length}} & \multicolumn{1}{|c|}{$\suspicion(\optSeq)$} & \multicolumn{1}{|c|}{\textbf{Error}} & \multicolumn{1}{|c|}{\textbf{Length}} & \multicolumn{1}{|c||}{$\suspicion(\optSeq)$} & \multicolumn{1}{|c|}{\textbf{Error}} & \multicolumn{1}{|c|}{\textbf{Error}} & \multicolumn{1}{|c|}{\textbf{Length}}& \multicolumn{1}{|c|}{$\suspicion(\optSeq)$}\\\hline
%		WM71 & $0.185$ & $0.335$ & $20$ & $-0.815$ & $0.255$ & $20$ & $-0.910$ & $0.160$ & $0.280$ & $20$ & $-0.884$\\\hline
%		WMOA & $0.185$ & & & & $0.260$ & $100$ & $-0.427$ & $0.160$ & $0.265$ & $20$ & $-0.938$ \\\hline
%		GP52 & $0.030$ & & & & $0.030$ & $100$ & $-0.413$ & $0.055$ & $0.115$ & $20$ & $-0.885$ \\\hline
%		GPOA & $0.030$ & & & & $0.055$ & $100$ & $-0.330$ & $0.055$ & $0.120$ & $20$ & $-0.903$ \\\hline
%		CABH & $0.162$ & $0.243$ & $500$ & $-0.174$ & $0.255$ & $500$ & $-0.179$  & $0.144$ & $0.278$ & $500$ & $-0.227$\\\hline
%		CAIM & $0.162$ & $0.240$ & $500$ & $-0.177$ & $0.259$ & $500$ & $-0.176$ & $0.144$ & $0.339$ & $500$ & $-0.227$ \\\hline
%		DRBH & $0.243$ & $0.300$ & $500$ & $-0.130$ & $0.273$ & $500$ & $-0.123$ & $0.248$ & $0.335$ & $100$ & $-0.401$ \\\hline
%		DRIM& $0.243$ & $0.298$ & $500$ & $-0.156$ & $0.303$ & $500$ & $-0.145$ & $0.248$ & $0.323$ & $100$ & $-0.389$ \\\hline
%	\end{tabular}}
%\end{table*}



%\begin{table}[!htb]
%	\centering
%	\caption{Test error rate for neural network learner. We also show the corresponding length of the training set and value of the detector function along with the baseline test error rate}~\label{tab:nnResults}
%	\resizebox{0.48\textwidth}{!}{%
%	\begin{tabular}{|l|r|r|r|r|}
%		\hline
%		\textbf{Name} & \textbf{Baseline} & \multicolumn{3}{|c|}{\textbf{Beam Search}} \\\cline{3-5}
%		& \multicolumn{1}{|c|}{\textbf{Error}} & \multicolumn{1}{|c|}{\textbf{Error}} & \multicolumn{1}{|c|}{\textbf{Length}} & \multicolumn{1}{|c|}{$\suspicion(\optSeq)$} \\\hline
%		WM71 & $0.160$ & $0.280$ & $20$ & $-0.884$\\\hline
%		WMOA & $0.160$ & $0.265$ & $20$ & $-0.938$ \\\hline
%		GP52 & $0.055$ & $0.115$ & $20$ & $-0.885$ \\\hline
%		GPOA & $0.055$ & $0.120$ & $20$ & $-0.903$ \\\hline
%		CABH & $0.144$ & $0.278$ & $500$ & $-0.227$\\\hline
%		CAIM & $0.144$ & $0.339$ & $500$ & $-0.227$ \\\hline
%		DRBH & $0.248$ & $0.335$ & $100$ & $-0.401$ \\\hline
%		DRIM & $0.248$ & $0.323$ & $100$ & $-0.389$ \\\hline
%	\end{tabular}}
%\end{table}

%We show average Alice's loss with respect to search budget for the logistic regression learner in Figure~\ref{fig:manWomanBudget}. As expected, Alice's loss gradually decreases as the search proceeds. But the reduction of loss slowly decreases. This reduction depends on the size of the camouflaged training set. The larger the budget, the more important it is to increase the search budget. 

%\begin{figure}[!htb]
%	\centering
%	\includegraphics[width=0.45\textwidth]{figures/CIFAR-100_1_7_1_inhomo_logistic_200000_10_50_set_lr_best_val_errors2.pdf}
%	\caption{Search Budget vs Alice's Error for WM71 using different training sizes for logistic regression learner}~\label{fig:manWomanBudget}
%\end{figure}

%We show the camouflaged training sets (of size 20) found for the image classification tasks in Figure~\ref{fig:manWomanTraining}. We also show some samples of the sensitive set here as well. It can be seen that no relation can be seen between the camouflaged training sets and the sensitive dataset. Thus it is really hard for any eavesdropping agent to figure out the actual illicit classification task even when she suspects something malicious is going on. 


%\begin{figure*}[!tbh]
%	\centering
%	\includegraphics[width=0.95\textwidth]{figures/cifar_oa.pdf}
%\caption{Camouflaged training set using oranges vs. apples (WMOA). 
%The secret task woman vs. man was shown in Figure~\ref{fig:sd}, while another camouflage training set using 7 vs. 1 was shown in Figure~\ref{fig:cts}.
%}~\label{fig:moreexamples2}
%\end{figure*}




%Our experimental results show the feasibility of training set camouflage. 
%We observe that Alice, using either NLP, beam search solver or uniform sampling, can find much better camouflage training sets than random and in many cases approach oracle.
%Keep in mind that Alice's solutions do not trigger Eve's suspicion function.
%This shows that such subterfuges are plausible in practice and can actually yield good results from Alice's point of view.

\begin{table}[htb]
	\centering

	\caption{Camouflage results for the CABH experiment with $m=20$}
	\label{tab:CABH}

	\resizebox{\textwidth}{!}{%
		\begin{tabular}{|l|l|l|l|}
			\hline
			\multicolumn{2}{|c|}{\textbf{Sample of Secret Set}} & \multicolumn{2}{|c|}{\textbf{Sample of Camouflaged Training Set}} \\\hline
			\multicolumn{1}{|c|}{\textbf{Class}} & \multicolumn{1}{|c|}{\textbf{Article}} & \multicolumn{1}{|c|}{\textbf{Class}} & \multicolumn{1}{|c|}{\textbf{Article}} \\\hline
			Christianity & $\ldots$Christ that often causes christians to be very & Baseball & $\ldots$The Angels won their home opener against the\\ 
			&  critical of themselves and other christinas. We$\ldots$ & &  Brewers today before 33,000+ 
			at Anaheim Stadium$\ldots$\\\cline{2-2}\cline{4-4}
			& $\ldots$I've heard it said that the accounts we have   & & $\ldots$ interested in finding out how I might be able\\
			& of Christs life and ministry in the Gospels were$\ldots$ & &  to get two tickets for the All Star game in Baltimore$\ldots$ \\\hline
			Atheism& $\ldots$This article attempts to provide a general  & Hockey & $\ldots$ user and not necessarily those could anyone post   \\
			& introduction to atheism. Whilst I
			have tried to be$\ldots$ & & the game summary for the Sabres-Bruins game.$\ldots$\\\cline{2-2}\cline{4-4}
			& $\ldots$Science is wonderful at answering most of our  & & $\ldots$Tuesday, and the isles/caps game is going into 
			\\
			& questions. I'm not the type
			to question scientific$\ldots$ & & overtime. what does ESPN do. Tom Mees says, "we$\ldots$\\\hline
		\end{tabular}}
\end{table}
%		& $(231,038)$ & $(275,535)$ & - & - \\\hline
%		25 & $0.672$ & $0.433$ & - & - \\
%		& $(229,039)$ & $(284,157)$ & - & - \\\hline
%		52 & $0.688$ & $0.390$ & - & - \\
%		& $(223,429)$ & $(288,583)$ & - & - \\\hline
%		69 & $0.798$ & $0.632$ & - & - \\
%		& $(227,243)$ & $(280,036)$ & - & - \\\hline
%		96 & $0.679$ & $\mathbf{0.337}$ & - & - \\
%		& $(217,095)$ & $(275,772)$ & - & - \\\hline
%		OA & $\mathbf{0.584}$ & $0.510$ & - & - \\
%		& $(235,536)$ & $(278,660)$ & - & - \\\hline
%		AO & $0.731$ & $0.531$ & - & - \\
%		& $(233,628)$ & $(278,976)$ & - & - \\\hline
%		BH & - & - & $\mathbf{0.638}$ & $\mathbf{0.681}$ \\
%		& - & - & $(278,397)$ & $(203,911)$ \\\hline
%		HB & - & - & $0.673$ & $0.684$ \\
%		& - & - & $(290,539)$ & $(212,123)$ \\\hline
%		IM & - & - & $0.676$ & $0.682$ \\
%		& - & - & $(271,315)$ & $(321,232)$ \\\hline
%		MI & - & - & $0.675$ & $0.683$ \\
%		& - & - & $(277,706)$ & $(210,645)$ \\\hline
%		AM & - & - & $0.676$ & $0.682$  \\
%		& - & - & $(286,292)$ & $(345,258)$ \\\hline
%		MA & - & - & $0.674$ & $0.682$ \\
%		& - & - & $(303,565)$ & $(211,582)$ \\\hline
%		MX & - & - & $0.675$ & $0.682$  \\
%		& - & - & $(298,501)$ & $(211,204)$ \\\hline
%		XM & - & - & $0.675$  & $0.683$ \\
%		& - & - & $(288,489)$ & $(327,451)$ \\\hline
%	\end{tabular}
%\end{table}

Figures~\ref{fig:example} shows the results of WMOA when Bob's learner is logistic regression and the solver is beam search $(m=20)$.
Visually, the camouflaged training set $D$ bears no resemblance to the secret training set $D_S$.
This is true for text camouflage experiments as well, where articles in the camouflaged training sets have no obvious semantic connection to the sensitive task. 
See Table~\ref{tab:CABH} for results on the text experiment CABH.
This is indeed bad news for human Eves: not only did camouflage fooled MMD detector, it will also likely fool human inspectors.

%\subsubsection{NLP Results}
As mentioned previously, Alice ran a separate experiment for the NLP solver.
Alice evaluates a further $m$ training sets as part of the rounding procedure for NLP.
Let $I$ and $N$ identify the index vector of all instances in the initial dataset and all other instances in the camouflage pool respectively. 
Also let, $I'$ and $N'$ represent the sorted sequence of $I$ and $N$ such that $b_{I'_i} \ge b_{I'_i+1}$ and $b_{I'_i} \ge b_{I'_i+1}$. Now we define,
$T_c=[I'_1,I'_2,\ldots,I'_{m-c},N'_1,N'_2,\ldots,N'_c]$.  
Here $c\in\mathbb{Z}: c\in[0,m]$. 
Thus $T_0=I'$ and $T_m=[N'_1,N'_2,\ldots,N'_m]$.
Alice evaluates the training sets $\cand_{T_c}$ for all values of $c$. 
Note that she does not need to re-evaluate $T_0$. Thus the camouflaged training set found by using NLP solver is:
\begin{align}
\argmin_{c\in\mathbb{Z}: c\in[0,m]}& ~~&&\frac{1}{\vert \val \vert} \sum_{(\tx, \ty)\in \val}\tloss(\hat{\theta}, \tx, \ty)\nonumber\\
\text{s.t.}& ~~&&\hat{\theta} = \argmin_{\theta \in \Theta} \sum_{(\bfx, y)\in\cand_{T_c}} \closs(\theta, \bfx, y) + \frac{\lambda}{2} \Vert \theta \Vert^2\nonumber\\
& &&\suspicion(\cand,\cand_{T_c}) < 0
\end{align}
We compare this result against the other two solvers ran from the same amount of time (after the initial run with budget $80,000$). 
For WMOA, GP96, CABH and DRBH the NLP solver took $15886$, $49555$, $40$ and $65$ seconds respectively to finish on an Intel(R) Core(TM) i7-7700T CPU @2.90GHz machine. The results are shown in Figure~\ref{fig:nlp}.

%\begin{table}[!htb]
%	\centering
%	\caption{Time Required to Run NLP}
%	\begin{tabular}{|c|r|}
%		\hline
%		Dataset & Time (seconds)\\\hline
%		WMOA & 15886.38 \\\hline
%		GP96 & 49555.30 \\\hline
%		CABH & 39.52 \\\hline
%		DRBH & 65.33 \\\hline
%	\end{tabular}
%\end{table}

%\begin{table}[!htb]
%	\centering
%	\caption{NLP results for $m=20$ for Logistic Regression Learner. Improvements are highlighted in bold.}
%	\begin{tabular}{|c|c|c|c|}
%		\hline
%		\textbf{Dataset} & \textbf{Solver} & \textbf{Starting Test Error Rate} & \textbf{Final Test Error Rate} \\\hline
%		& NLP & 0.280 & 0.305  \\\cline{2-4}
%		WMOA & Beam Search & 0.280 & 0.300  \\\cline{2-4}
%		& Uniform Sampling & 0.340 & 0.325  \\\hline
%		& NLP & 0.075 & \textbf{0.070} \\\cline{2-4}
%		GP96 & Beam Search & 0.075 & \textbf{0.055} \\\cline{2-4}
%		& Uniform Sampling & 0.120 & 0.120 \\\hline
%		& NLP & 0.406 & 0.406 \\\cline{2-4}
%		CABH & Beam Search & 0.406 & 0.406 \\\cline{2-4}
%		& Uniform Sampling & 0.437 & 0.437 \\\hline
%		& NLP & 0.343 & \textbf{0.340} \\\cline{2-4}
%		DRBH & Beam Search & 0.343 & 0.343 \\\cline{2-4}
%		& Uniform Sampling & 0.375 & 0.375 \\\hline
%	\end{tabular}
%\end{table}

\begin{figure}[htb]
	\centering
	\centering
	\includegraphics[width=0.3\textwidth]{figures/nlp_lr_20.pdf}
	\caption{NLP results for $m=20$ for Logistic Regression Learner. Both beam search and uniform sampling solvers are run for the same amount of time as the NLP solver(after the initial $80,000$ budget). }~\label{fig:nlp}
\end{figure}


\subsection{Discussion}
Our experimental results show that training set camouflage is indeed a plausible threat.
We present three approaches to solve the optimization problem.
We observe that beam search largely outperforms uniform sampling.
%This suggests that our simple relaxation and rounding strategy in NLP needs improvement.
It should also be noted that the NLP solver can be used to slightly improve the solution of the input dataset.
%It should also be noted that the solutions found by NLP may not be feasible (i.e., $\suspicion(\cand,\optSeq)>0$).
%But this scenario did not occur during our experiments.
All these observations combined with the fact that beam search is also applicable to a wider range of learners (non-convexity prevents the application of KKT condition), makes beam search the preferred solver for Alice.

%\begin{figure}[htb]
%	\centering
%	\includegraphics[width=0.48\textwidth]{figures/diff_size_error_GP52.pdf}
%	\caption{Test error rate for different training set sizes. For both logistic regression and ANN we show the results for beam search on the GP52 dataset.}~\label{fig:diffSize}
%\end{figure}

%\begin{figure}[htb]
%	\centering
%	\includegraphics[width=0.48\textwidth]{figures/gen_error_lr_beam_search.pdf}
%	\caption{Secret set and Test set error rate for logistic regression using Beam Search. For image and text datasets we show results for $\trainSize=20$ and $\trainSize=500$ respectively for brevity.}~\label{fig:generalizationError}
%\end{figure}

We note that $\mmd$ is stronger with larger sample sizes.
It will be harder for Alice to fool Eve given a large camouflage pool $C$ and also if she is forced to select a large camouflaged training set $D$. 
$\mmd$ is also stronger with smaller feature dimensions~\cite{gretton2012kernel}.
Also, it is harder for Alice to fool Eve if she increases the value of $\alpha$.
Since $\alpha$ is the upper bound of the probability of the Type I error for the null hypothesis i.e., the camouflage pool and camouflaged training set come from the same distribution, increasing $\alpha$ allows Eve to become more suspicious.
Moreover, it is also possible for Eve to use other detection functions. 
The application of training set camouflage framework will remain the same regardless. 


%We designed the experiments so that Alice needs to teach the same secret task (e.g. woman vs. man) to Bob using two different cover tasks (e.g. 7 vs 1, and orange vs. apple).
%Interestingly, which cover task was used does not matter much.
%Conversely, Alice also needs to teach different secret tasks (e.g. woman vs. man, and gun vs. phone) to Bob using the same cover task (e.g. orange vs. apple). Alice also succeeds in this task to some degree.
We note that camouflage seems easier for Alice to do if the cover task is in fact somewhat confusable, presumably because she can generate different decision boundaries by picking from overlapping camouflage items.
This can be imagined easily in the 2D case with two overlapping point clouds forming the cover task.
In such a scenario any separable secret task (no overlap between the secret task instances) can be taught to Bob by Alice. 
One interesting open question is whether there is a \textit{universal} cover task for all secret tasks (they must use the same feature representation, of course).

As mentioned previously, Bob fixed his learning hyperparameters (e.g., regularization parameter of the logistic regression).
This was done for speed.
However, nothing prevents Bob from using cross validation~\cite{kohavi1995study}. 
Cross validation is popular technique used in machine learning where the learner is trained multiple times on different subsets of the whole training set to tune the hyperparameters of the learner.
Alice would simply emulate the same cross validation while optimizing the camouflaged training set.
This can be easily done in beam search and uniform sampling, at the cost of more computation.
This also suggests that these two solvers are much useful in practice than NLP.

Also, the loss function $\ell$ used by Alice and Bob is the same, as seen in the upper and lower optimization problems in~\eqref{eq:MMDConstraint}.
It is straightforward to allow different losses.  For example, Bob may learn with the logistic loss since it is a standard learner, while Alice may use 0-1 loss to directly optimize Bob's accuracy.

%Moreover, we note that the assumption of Eve's detection function being known to Alice can be relaxed as well. If Alice does not have access to said detection function then it is possible for her to generate a surrogate of that function by probing Eve with multiple datasets (while not training Bob). Once Alice is confident about the surrogate function, she can again apply the same techniques to generate the camouflaged training set. We leave out this discussion for future work.

It should also be noted that the training set camouflage can also be extended to cross modality correspondence, e.g., use an image camouflage pool with feature vectors of size $2048$ while the secret classification task is to classify text articles. 
In such a case Alice and Bob can decide beforehand to use the $2048$ most frequent words in the text articles to form bag of word (BOW) feature vectors for the secret classification task.

